SafeDrug: Dual Molecular Graph Encoders for Recommending Effective and Safe Drug Combinations

Medication recommendation is an essential task of AI for healthcare. Existing works focused on recommending drug combinations for patients with complex health conditions solely based on their electronic health records. Thus, they have the following limitations: (1) some important data such as drug molecule structures have not been utilized in the recommendation process. (2) drug-drug interactions (DDI) are modeled implicitly, which can lead to sub-optimal results. To address these limitations, we propose a DDI-controllable drug recommendation model named SafeDrug to leverage drugs' molecule structures and model DDIs explicitly. SafeDrug is equipped with a global message passing neural network (MPNN) module and a local bipartite learning module to fully encode the connectivity and functionality of drug molecules. SafeDrug also has a controllable loss function to control DDI levels in the recommended drug combinations effectively. On a benchmark dataset, our SafeDrug is relatively shown to reduce DDI by 19.43% and improves 2.88% on Jaccard similarity between recommended and actually prescribed drug combinations over previous approaches. Moreover, SafeDrug also requires much fewer parameters than previous deep learning-based approaches, leading to faster training by about 14% and around 2x speed-up in inference.

==> cover_letter/AAAI21_review.tex <==
\section{Reviewer \#1}

\noindent {\bf Summary} 

Please summarize the main claims/contributions of the paper in your own words. (Do not provide any review in this box)
In this paper, the authors proposed a novel DDI-controllable drug recommendation model named “SafeDrug”. The main contribution of this paper is to design the global MPNN encoder and local bipartite encoder to leverage the structure information of drugs. The experimental results show that incorporating drug structure information can improve the performance of drug recommendation.

\noindent {\bf Novelty} 

How novel is the paper?
Paper contributes some new ideas

\noindent {\bf Soundness} 

Is the paper technically sound?
The paper has major technical flaws, necessitating another review after corrections

\noindent {\bf Impact} 

How important is the paper likely to be, considering both methodological contributions and impact on application areas?
The paper will have low overall impact

\noindent {\bf Clarity} 

Is the paper well-organized and clearly written?
Fair: paper is somewhat clear, but important details are missing or confusing, which hurts readability

\noindent {\bf Evaluation} 

Are claims well supported by experimental results?
Good: Experimental results are sufficient, though more analysis would significantly add support to the claims

\noindent {\bf Resources} 

How impactful will this work be via sharing datasets, code and/or other resources? (It may help to consult the paper’s reproducibility checklist.)
Fair: some may find shared resources useful in future work

\noindent {\bf Reproducibility}

Would the experiments in the paper be easy to reproduce? (It may help to consult the paper’s reproducibility checklist.)
Poor: e.g., experimental setup details are incomplete/unclear, and code/data are not available to aid reproducibility

\noindent {\bf Reasons to Accept} 

Please describe the paper’s key strengths.
The proposed method can extract rich structural information from drug molecules for the better representation of drugs. Specifically, two structure embedding modules are applied to encode different types of structure information. The proposed local bipartite encoder is simple but effective.

\noindent {\bf Reasons to Reject} 

Please describe the paper’s key weaknesses.
The authors preprocessed the datasets in a different way from previous baselines. The size of drug set is reduced by grouping similar drugs. Considering that similar drugs are grouped, the reviewer wonders how to apply the structure information of these grouped drugs and how to evaluate the accuracy of predictions of these grouped drugs.

The authors extracted substructures by using the synthetically accessible bonds. However, fragmenting molecules using these bonds can be unrelated with the local functionality. In other words, the pharmacophore of drugs may be broken and assigned to multiple groups.

The paper claims that the local bipartite encoder has good interpretability. But the paper doesn’t provide detailed analysis towards the interpretability.

The F1 evaluation is based on the ground-truth prescribed drugs. The only way to reduce DDI rates from ground-truth drugs is to either not predict ground-truth drugs (i.e., scarifying the recall) and/or predict additional drugs not in the ground-truth (i.e., scarifying jaccard). Based on the results, both of the two cases happened. Then the key point is to justify whether this is clinically useful and sensible: what is the point not to prescribe drugs that are supposed to treat a disease, and what is the point to prescribe drugs that the patients do not need.

\noindent {\bf Detailed Comments} 

Please provide other detailed comments and constructive feedback.
The authors preprocessed the dataset in a different way from previous baselines. The paper doesn’t include the details about the preprocessing of procedure, but the data statistics table shows that the number of procedures is less than the statistics provided by GAMENet. If the procedure information is preprocessed, it is suggested to include these details into the paper.

Besides, according to the paper, similar drugs are grouped together by ATC code to reduce the size of drug set. However, these grouped drugs should have different structures. But the paper doesn’t include the details about what kinds of structures are used to represent those grouped drugs and how to measure the DDI values of these grouped drugs and the predicted accuracy of these grouped drugs.

To show that the proposed local bipartite encoder can capture pharmacophore or local functionality information of drugs, it is suggested to add more analysis towards the interpretation of the learned weight for bipartite graph. For example, the learned local bipartite encoder may be able to be interpretated by checking whether the substructures with large weight values are the pharmacophores of corresponding drugs or not, or checking whether the learned patient embedding mf can capture important substructures for some diseases. The paper claimed that the local bipartite encoder has good interpretability, so it is suggested to add the analysis towards interpretability into the paper.

The paper claims that the proposed model can recommend safe drugs with lower DDI values than the dataset. However, as the paper mentioned, lower DDI value can be resulted from fewer drugs. Considering that fewer drugs may indicate less effectiveness, the reviewer wonders whether it is possible to prove that the recommended drugs with lower DDI values can at least maintain their efficacy.

\noindent {\bf QUESTIONS FOR THE AUTHORS} 

Please provide questions for authors to address during the author feedback period. (Please number them)

(1) It is suggested to include more details about the grouping of similar drugs and the substructures used to represent the grouped drugs. How many substructures are extracted by BRICS? Is it possible to extract substructures related to the functionality of drugs?

(2) It is suggested to add more details about the dataset preprocessing, such as the reason why the number of procedures in this paper (962) is significantly less than the number in GAMENet (1426).

(3) It is suggested to add more analysis towards the interpretability of local bipartite encoder.

(4) Is it possible to evaluate the efficacy of recommended drugs with lower DDI value?
13. {Ethical Considerations} Please highlight any ethical considerations that must be considered before a final decision (it may help to consult the paper’s ethics statement, if provided)
None

\noindent {\bf OVERALL SCORE}

4 - Reject


\section{Reviewer \#2}

\noindent {\bf Summary} 

Please summarize the main claims/contributions of the paper in your own words. (Do not provide any review in this box)
The author propose a machine learning method for drug recommendation based on drug molecule structures. A unique feature of the method is to encode the connectivity and functionality of drug molecules. The designed loss controller makes it possible to provide safe drug combinations.

\noindent {\bf Novelty} 

How novel is the paper?
Paper contributes some new ideas

\noindent {\bf Soundness} 

Is the paper technically sound?
I have not checked all details, but the paper appears to be technically sound

\noindent {\bf Impact} 

How important is the paper likely to be, considering both methodological contributions and impact on application areas?
The paper will have low overall impact

\noindent {\bf Clarity} 

Is the paper well-organized and clearly written?
Fair: paper is somewhat clear, but important details are missing or confusing, which hurts readability

\noindent {\bf Evaluation} 

Are claims well supported by experimental results?
Poor: The experimental design is flawed and unconvincing

\noindent {\bf Resources} 

How impactful will this work be via sharing datasets, code and/or other resources? (It may help to consult the paper’s reproducibility checklist.)
Fair: some may find shared resources useful in future work

\noindent {\bf Reproducibility} 

Would the experiments in the paper be easy to reproduce? (It may help to consult the paper’s reproducibility checklist.)
Good: e.g., code/data available, but some details of experimental settings are missing/unclear

\noindent {\bf Reasons to Accept} 

Please describe the paper’s key strengths.
The proposed method achieved high accuracy.

\noindent {\bf Reasons to Reject} 

Please describe the paper’s key weaknesses.
The problem setting is not realistic. Medical doctors do not take into account chemical structures of drugs in practice. Nobody will use chemical structure-based methods for medical treatment.

\noindent {\bf Detailed Comments} 

Please provide other detailed comments and constructive feedback.
The author propose a machine learning method for reliable and safe drug recommendation, but the problem setting is not realistic. Medical doctors select drugs based on their mode-of-action and indications in practice. Medical doctors do not take into account chemical structures of drugs in practice. Nobody will use chemical structure-based methods for medical treatment.

The authors say that pharmacological properties of a drug is largely determined by its chemical structure. Chemical structure is very important in drug development processes such as lead discovery and structure optimization. However, chemical structures are not taken into account in clinical practice.

There are many previous works on computational methods (including supervised learning and unsupervised learning) for drug combination/interaction prediction. There is no comparison with previous works with the same goal. For example, see the following papers:
- PLoS Comput. Biol. 7, e1002323, 2011
- Mol. Syst. Biol. 8, 592, 2012
- J. Chem. Inf. Model. 55(12), 2705–2716, 2015

\noindent {\bf QUESTIONS FOR THE AUTHORS} 

Please provide questions for authors to address during the author feedback period. (Please number them)
The authors classified drugs by ATC codes, but ATC codes have a hierarchy. Which level are used?

\noindent {\bf OVERALL SCORE}

3 - Clear reject

==> cover_letter/WWW21_review.tex <==
\section{Reviewer \#1}

\noindent {\bf Relevance to the Web Conference:}

-1: (Not relevant)
This paper, despite its merits, only has tangential relevance to the Web, at best. It describes a drug recommendation algorithm. The authors ground the necessity for an ML approach to drug recommendation in the fact that "massive biomedical data [is] available on the web." (p.1). But this is about as far as the paper goes in establishing relevance to the conference. Given that this is also the Web and Society track of the Web Conference, I am really struggling to see how this paper could fit in.

\noindent {\bf Overall evaluation:}	

-2: (Reject) 

\noindent {\bf Summary:}

The paper provides the description of an algorithm for drug recommendation, aimed at minimizing drug-drug interactions. The algorithm uses RNNs to generate a both a patient representation and a drug representation the former based on patient histories, and the latter on the drug's molecular structure. The authors provide experimental evidence that their algorithm improves on what they identify as the state of the art in the field.

\noindent {\bf Originality:}

3: (Creative: Only a few people in our community would have put these ideas together)
My expertise here is rather limited, but this seems like a creative use of neural networks.

\noindent {\bf Potential impact:}

2: (Limited: Impact limited to improving the state-of-the-art for the problem being tackled)
It is difficult for a non-specialist to evaluate impact of a drug recommendation algorithm. An educated guess would lead me to believe that drug recommendation is very difficult to do in practice, likely due to issues that have little to do with ML per se (e.g. liability and concern about overfitting).

\noindent {\bf Reproducibility:}

2: (Some but not all code, data or the details of the experimental setup are made available)
The authors present a model that seems reasonably straightforward to reproduce, despite its complexity.

\noindent {\bf Quality of execution:}

3: (Reasonable: Generally solid work, but certain claims could be justified better)
Again, an educated guess since I am not qualified to assess pharmacological AI, but I was able to follow the paper seen from an ML lens.

\noindent {\bf Quality of presentation:}

3: (Reasonable: Understandable to a large extent, but parts of the paper need more work)
See above.

\noindent {\bf Adequacy of citations:}

2: (Reasonable: Coverage of past work is acceptable, but a few papers are missing)
See above.

\noindent {\bf Ethics:}

1: (No)
No ethical concerns. The paper uses what appears to be a canonical dataset in the field, and the model's recommendations do not appear to be currently used in medical decision making. I would have concerns about explainability and verifiability of the model's reasoning if these recommendations *were* being used when making real clinical decisions, but these are out-of-scope to this paper.

\noindent {\bf Strengths:}

+ creative use of modern neural networks methods.
+ important problem that is likely on the list of priorities for the healthcare sector.

\noindent {\bf Weaknesses:}

- not suited to the Web Conference.

\noindent {\bf Reasons to accept:}

\noindent {\bf Reasons to reject:}

The biggest reason to reject is the poor fit with the conference. I had to re-read the CfP a few times to make sure I did not misunderstand something. The most relevant paragraph describes the requirements for health research at the conference:

"Health on the Web: New this year, the Web and Society track also includes research related to health on the Web (previously a separate track) that brings together advances in Internet-related computer science with direct benefits to the medical and health domains. Relevant research includes advances in computer science as applied to health or medicine on the Web, significant advances in health, utilizing existing state-of-the-art computational techniques, and reports on significant lessons learned from a real-world deployment of medicine or health-related Web technology. Of particular interest is research showing how the Web can improve individual and public or provide better healthcare delivery. Submissions related to the Covid-19 pandemic are especially welcome."

The submission does indeed show how advances in computer science could have direct benefits to the medical domain. However, I do not understand which of these advances are *Internet*-related. In my view, this paper would be better suited to a general-purpose ML conference (e.g. AAAI), one focused on Artificial Neural Networks (e.g. NeurIPS), or one of (what I am sure are) many medical AI conferences.

\section{Reviewer \#2}

\noindent {\bf Relevance to the Web Conference:}

1: (Relevant)

\noindent {\bf Overall evaluation:}	

2: (Accept)

\noindent {\bf Summary:}

In this paper, the authors propose a novel SafeDrug model for the problem of safe drug recommendations. Our model extracts rich molecule structure information from the web and introduces dual (global and local) molecular structural encoders to help the drug recommendation
task.

\noindent {\bf Originality:}

3: (Creative: Only a few people in our community would have put these ideas together)

\noindent {\bf Potential impact:}

3: (Broad: Could help ongoing research in a broader research community)

\noindent {\bf Reproducibility:}

3: (All code, data, and the details of the experimental setup are made available)

\noindent {\bf Quality of execution:}

4: (Thorough: The approach is well-justified and all the claims are convincingly supported)

\noindent {\bf Quality of presentation:}

4: (Lucid: Very well written in every aspect, a pleasure to read, easy to follow)

\noindent {\bf Adequacy of citations:}

3: (Comprehensive: Can't think of any important paper that is missed)

\noindent {\bf Ethics:}

1: (No)
No ethical concerns

\noindent {\bf Strengths:}

\begin{itemize}
    \item SafeDrug uses a global message passing neural network (MPNN) module and a local bipartite learning module to fully encode the connectivity and functionality of drug molecules.
    \item The authors claim that SafeDrug beats state of the art baselines with a significant reduction on DDI by 19.43\%, improvement over Jaccard similarity between the recommendation and the real prescription by 2.88\% and F1-score by 2.14\%
    \item SafeDrug trains faster compared to other states of the art methods, as mentioned.
\end{itemize}

\noindent {\bf Weaknesses:}

The paper lacks an in-depth conclusion with the possible improvements and its future scope.

\section{Reviewer \#3}

\noindent {\bf Relevance to the Web Conference:}

-1: (Not relevant)

\noindent {\bf Overall evaluation:}	

-2: (Reject)

\noindent {\bf Summary:}

This work presents SafeDrug, a drug recommender system designed to provide safe drugs combinations by taking into consideration molecular structure and patients' medical history.

Overall, the paper is well motivated: it mentions how existing work often take into account previous medication, but fail to how drugs interact at a molecular level, or are often implicitly encoded with interpretable mechanisms. Empirical results indicate that the proposed method improves over other techniques.

Unfortunately, this work, while of good quality, doesn't follow into the scope of The Web Conference. No web data or processes are modeled anywhere in the paper; in fact, this work does not use any unstructured free form text that could be distributed on web platforms. I would encourage the authors to submit this work to a venue that is better suited to this topic.

\noindent {\bf Originality:}

2: (Conventional: Rather straightforward, a number of people could have come up with this)

\noindent {\bf Potential impact:}

2: (Limited: Impact limited to improving the state-of-the-art for the problem being tackled)

\noindent {\bf Reproducibility:}

2: (Some but not all code, data or the details of the experimental setup are made available)

\noindent {\bf Quality of execution:}

3: (Reasonable: Generally solid work, but certain claims could be justified better)

\noindent {\bf Quality of presentation:}

3: (Reasonable: Understandable to a large extent, but parts of the paper need more work)

\noindent {\bf Adequacy of citations:}

2: (Reasonable: Coverage of past work is acceptable, but a few papers are missing)

\noindent {\bf Ethics:}

1: (No)
N/A

\noindent {\bf Strengths:}

Well motivated

\noindent {\bf Weaknesses:}

Not relevant to the conference

==> cover_letter/abstract.tex <==
\begin{abstract}
Medication recommendation is an essential task for predictive health.
Most of the recently proposed medication recommendation algorithms focused on  recommending drug combinations for patients with complex health conditions solely based on their  electronic health records, and thus have the following limitations: (1) There are other important data such as {\em drug molecule structures}, which can help augment drug recommendation but have not been utilized by existing models. (2) Existing works model drug-drug interactions (DDI) implicitly and can lead to variable DDI rates or sub-optimal recommendation accuracy. 

To address these limitations, we propose a DDI-controllable drug recommendation model named \method to leverage drugs' molecule structures and model DDIs explicitly.
\method is equipped with a global message passing neural network (MPNN) module and a local bipartite learning module, to fully encode the connectivity and functionality of
drug molecules. \method also has a  controllable loss function to effectively control DDI level in the recommended drug combinations.  We experimentally evaluate \method on a real-world benchmark medication recommendation dataset and demonstrate  that  \method outperforms existing medication recommendation models. Compared with the best baselines, \method reduces DDI by $19.43$\% and improves $2.88$\% on Jaccard similarity between  recommended and actually prescribed  drug combinations over previous approaches and $2.14$\% on F1-score. Moreover, \method requires much fewer parameters than previous deep learning drug recommendation approaches, while leads to faster training by about 14\% and around $2\times$ speed-up in inference. 
\end{abstract}

==> cover_letter/conclusion.tex <==
\section{Conclusion} In this paper, we propose a novel
\method model for the problem of safe drug recommendation. Our model
extracts rich molecule structure information from the web and introduces dual (global and local) molecular structural encoders to help the drug recommendation task. We design adaptive loss controller, which enables the model
to provide reliable and safe drug combinations. The model is evaluated on a
public {\em MIMIC-III} dataset, where we beat state of the art baselines with a significantly reduction on DDI by 19.43\%, improvement over Jaccard similarity between the recommendation and the real prescription by 2.88\% and F1-score by 2.14\%. Our \method model is also reported to have fewer parameters than state of the art methods with faster training and almost $2\times$ speedup in inference.
% rate and higher accuracy.
% \js{expand the conclusion w/ a bit more details such as performance results and improvement percentage}

==> cover_letter/cover_letter.tex <==
\section{Main Reason for Previous Rejection}
There are three reviewers (in theWebConf 2021): one reviewer suggests acceptance, while the other two did not provide reviews due to their concern about our manuscript's relevance to the web conference. There are two reviewers (in the AAAI 2021): The first reviewer encourages us to add more processing steps, more details for datasets, and he also questions on the experimental settings. The second reviewer thinks the motivation of the paper is limited, and he believes that a real doctor will not consider drug molecule structures when making prescriptions. 

% Some of the reviewers are concerned about the fit to TheWebConf 2021, and they think the submission lacks the relevance to the web.

\section{New Changes}
From the AAAI 2021 submission, the paper changed a lot. We improve the writing thoroughly, so as to make it more understandable. We add more contents to the paper, including the dataset descriptions, processing steps, metric standard deviations, hypothesis testing results, new baseline method and additional experiments.

For the experimental setting, we actually follow many newly published works, such as \cite{shang2019gamenet,zhang2017leap}. The dataset we used spans several years and includes many doctors' practice. In fact, it is a benchmark dataset for drug recommendation and the setting is also standard in the area. In terms of the motivation, real doctors have no time and also are unable to use drug molecule information for better prescription, that is why we want to develop a computational method that can use the computer power to process useful data sources for more accurate and effective drug recommendations. We aim to ease the doctors' effort while providing better clinical service for patients.

From the WebConf 2021 submission, though some of them are concerned about fitting to CFP, the reviewers do not raise any major concern to the content itself. We, therefore, did not change the content too much. The changes are mostly structure-wise. Here are the changes: 

First, due to space limitation, we remove the notation Table~1; we move the Algorithm~1 to Appendix; we move the dataset processing steps, implementation details, experimental settings, and the last two experiments to Appendix.

Then, we also made minor changes to the main text to make it more readable. The changes can be found in all sections, including Abstract and Introduction. For example, in subsection ``Longitudinal Patient Representation", we simplify the original expression (During a clinical visit, doctors
would first \textit{diagnose} the diseases and then apply therapeutic
\textit{procedures}. Based on these two steps, the doctors are
ready to prescribe drugs. In this work, the patient's health condition is also extracted based on both \textit{diagnosis} and \textit{procedure} information.) into a simpler and clearer sentence (From longitudinal EHR data, patient health can be encoded by their diagnosis and procedure information.)

==> cover_letter/experiment.tex <==
\section{Experiments} 
In the experiment, we comprehensively evaluate our \method model by answering the following five questions:

\vspace{0.5mm} \textbf{Q1:} How does \method perform in general
compared to \\ \indent \indent \indent state-of-the-art  baselines?

\vspace{0.5mm}
\textbf{Q2:} Is our model computationally efficient?

\vspace{0.5mm}
\textbf{Q3:} Does the model robust? How can we make the result safe  \\ \indent 
\indent  \indent and controllable?

\vspace{0.5mm}
\textbf{Q4:} In which case can our model work well, where and why\\ \indent \indent
\indent does \method fail?

\vspace{0.5mm}
\textbf{Q5:} What is the benefit of bipartite mask $\bm{H}$? How to interpret?

\subsection{Experiment Setup}\label{sec:setting}



\smallskip
\noindent
\textbf{Dataset.} The experiments are carried out on \textit{MIMIC-III} \cite{johnson2016mimic}.
This dataset
% \footnote{https://mimic.physionet.org/} 
is publicly available with
over 40,000 patients who stayed in intensive care unit (ICU) in the Beth Israel
Deaconess Medical Center for over 11 years. It consists of 50,206 medical
encounter records. % that associated with 6,695 distinct diseases and 4,127
% drugs.
% \textit{Sutter} is from Sutter Palo Alto Medical Foundation (PAMF) consists of
% 18-years longitudinal medical records of 258,000 patients between age 50 and
% 90. It contains 2,415,414 medical en-counters
% records.
% associated with 8,359 distinct diseases and 7,516 drugs.
We filter out the patients with only one visit. 
Diagnosis, procedure and medication information is initially documented in ``DIAGNOSES\_ICD.csv", ``PROCEDURES\_ICD.csv" and ``PRESCRIPTIONS.csv" in the original MIMIC sources. We extract them separately and then merge these three sources by patient id and visit id. After the merging, diagnosis and procedure are ICD-9 coded, and they will be transformed into multi-hot vectors before training. We extract the DDI information by Top-40 severity types from TWOSIDES \cite{tatonetti2012data}, which are reported by ATC Third Level codes. This paper then transforms the NDC drug codings to the same ATC level codes for integration, and in the implementation, we also average the drug-level MPNN embeddings and aggregate the substructures for the corresponding ATC Third level code. Basic statistics of the post-processed data is
reported in Table~\ref{tb:mimic}.

\begin{table}[h!] \caption{Data Statistics}
\centering
	\begin{tabular}{l|c} \toprule \textbf{Items} & \textbf{Size} \\ \midrule total
		\# of visits & 14,995 \\ total \# of patients & 6,350 \\ diag. / prod. /
		med. space size & 1,958 / 1430 / 131 \\ % 	procedure code set & 962 \\
		% 	medication set & 131 \\
		avg. / max \#  of visits & 2.37 / 29 \\ % 	max of visits & 29 \\
		avg. / max \#  of diagnoses per visit & 10.51 / 128 \\ % 	max of diagnoses per
		% visit & 128 \\
		avg. / max \#  of procedures per visit & 3.84 / 50 \\ % 	max of procedures per
		% visit & 50 \\
		avg. / max \#  of medicines per visit & 11.44 / 65 \\ % 	max of medicines per visit
		% & 65 \\
		total \# of DDI pairs & 448 \\
		total \# of substructures & 491 \\
\bottomrule \end{tabular}
	\label{tb:mimic} \end{table}

\smallskip
\noindent
\textbf{Baselines.} We compare \method with the following
baselines. To carry out fair
comparison, we also use 64 hidden units or 64-dim embedding tables for all the
modules in the baselines. \begin{itemize} % \item \textbf{Repeat.} This method
	% will assign the same recommendation in the last visit as the recommended
	% result in this visit and it is free from learning.
	\item \textbf{Logistic Regression (LR).} This is an instance-based classifier
	with $L_2$ regularization. We directly feed the concatenated multi-hot diagnosis and
	procedure vector as the feature, and medication vector as the target. The
	model is implemented by \textit{scikit-learn} with One-vs-Rest classifier, 500 maximum iteration, LBFGS algorithm as solver.

    \item
	\textbf{Ensemble Classifier Chain (ECC)} \cite{read2009classifier}. Classifier chain (CC) is a popular multi-label classification approach, which feeds previous classification results into the latter classifiers. We implement a 10-member ensemble of CCs also by \textit{scikit-learn}, where each CC consists of a dependent series of logistic regression classifiers with max iteration at 500 and LBFGS as optimizer.
	
	\item \textbf{RETAIN} \cite{choi2016retain} is an entirely temporal based
	method. It utilizes a two-level RNN with reverse time attention to model
	the longitudinal information. Following the original paper \cite{choi2016retain}, we choose two 64-dim GRUs as the implementation of two-level RNN with dropout rate at 0.5 for the output embedding. Adam is used as the optimizer with learning rate at $5\times 10^{-4}$ for RETAIN and other deep learning baselines.

	\item \textbf{LEAP} \cite{zhang2017leap} is a
	sequential decision making algorithm. It treats drug recommendation as a
	sentence generation task and recommend drugs one at a time. LEAP is also implemented by 64-dim GRU as the feature encoder. However, we choose droput rate at 0.3 between two layers, as 0.3 works better than 0.5 in the validation set. Particularly, since LEAP and DMNC are sequence-based models, we set 20 as their max drug combination size.
	
	\item \textbf{DMNC} \cite{le2018dual}. DMNC builds the drug recommendation model on differentiable neural computer (DNC). It models the diagnosis and procedure sequences by multi-view learning and uses a memory augmented neural networks (MANN). We use 64-dim embedding tables to represent medical codes, design 1-head, 1-layer, 16-cell DNC encoder using {\em dnc} package, and a 64-dim GRU decoder.

	\item \textbf{GAMENet} \cite{shang2019gamenet}. GAMENet is a recent work.
	This method also adopts memory augmented neural networks and stores
	historical drug memory records as references for future prediction. We use the same suit of hyperparameters reported from the original paper \cite{shang2019gamenet}: expected DDI rate at 0.05, initial annealing temperature at 0.85, mixture weights $\pi=[0.9, 0.1]$ and also use 64-dim embedding tables and 64-dim GRU as RNN. We find the hyperparameter works well in validation set, so we keep it for test.
\end{itemize}



\smallskip
\noindent
\textbf{Evaluation Metrics.}
We use the following performance metrics.
\begin{itemize} [leftmargin=*]
    \item \textbf{DDI rate} (smaller is better) for patient $j$ is calculated as below, \begin{equation}
\mathrm{DDI}_j = \frac{\sum^{V_j}_{t=1}\sum_{k, l\in \{i:~\hat{\bm{m}}^{(t)}_{j,i}=1\}} \bm{1}\{\bm{D}_{kl}=1\}}{\sum^{V_j}_{t=1}\sum_{k, l\in \{i:~\hat{\bm{m}}^{(t)}_{j,i}=1\}}1}, \notag
\end{equation} 
where $V_j$ denotes the total number of visits of the $j$-th patient, $\hat{\bm{m}}^{(t)}_j$ represents the predicted drug combination during  the $t$-{th} visit of patient $j$, $\hat{\bm{m}}^{(t)}_{j,i}$ denotes the $i$-th element of $\hat{\bm{m}}^{(t)}_j$, $\bm{D}$ is the DDI matrix (defined in Section~\ref{sec:notation}) and $\bm{1}\{\cdot\}$ is an indicator function, which returns 1 when the expression in $\{\cdot\}$ is true, otherwise 0. 
\item \textbf{The Jaccard coefficient} (higher is better) for patient $j$ at the $t$-th visit is calculated as follows,
\begin{equation}
    \mathrm{Jaccard}_j^{(t)} = \frac{|\{i:~\bm{m}_{j,i}^{(t)}=1\}\cap \{i:~\hat{\bm{m}}_{j,i}^{(t)}=1\}|}{|\{i:~\bm{m}_{j,i}^{(t)}=1\}\cup \{i:~\hat{\bm{m}}_{j,i}^{(t)}=1\}|},
\end{equation}
where ${\bm{m}}^{(t)}_j$ is the ground-truth drug combination during  the $t$-{th} visit of patient $j$, and ${\bm{m}}^{(t)}_{j,i}$ is the $i$-th element. $|\cdot|$ denotes the cardinality, $\cap$ is set interaction and $\cup$ is set union operation. Then, the Jaccard coefficient for one patient $j$ is by taking the average over her/his visits ($V_j$ is the total number of visits of patient $j$),
\begin{equation}
    \mathrm{Jaccard}_j = \frac{1}{V_j}\sum_{t=1}^{V_j}\mathrm{Jaccard}_j^{(t)},
\end{equation}
\item \textbf{The F1 score} (higher is better) is  the harmonic mean of precision and recall. For patient $j$ at visit $t$, the Precision, Recall, F1 are calculated by
\begin{equation}
    \mathrm{Precision}_j^{(t)} = \frac{|\{i:~\bm{m}_{j,i}^{(t)}=1\}\cap \{i:~\hat{\bm{m}}_{j,i}^{(t)}=1\}|}{ |\{i:~\hat{\bm{m}}_{j,i}^{(t)}=1\}|}
\end{equation}
\begin{equation}
    \mathrm{Recall}_j^{(t)} = \frac{|\{i:~\bm{m}_{j,i}^{(t)}=1\}\cap \{i:~\hat{\bm{m}}_{j,i}^{(t)}=1\}|}{ |\{i:~{\bm{m}}_{j,i}^{(t)}=1\}|}
\end{equation}
\begin{equation}
    \mathrm{F1}_j^{(t)} = \frac{2}{\frac{1}{\mathrm{Precision}_j^{(t)}}+\frac{1}{\mathrm{Recall}_j^{(t)}}}
\end{equation}
The F1 score for one patient $j$ is by taking the average over her/his visits,
\begin{equation}
    \mathrm{F1}_j = \frac{1}{V_j}\sum_{t=1}^{V_j}\mathrm{F1}_j^{(t)},
\end{equation}
\item \textbf{Precision Recall Area Under Curve (PRAUC)} (higher is better). To compute the PRAUC, we  treat the drug recommendation as an information retrieval problem. The PRAUC value for patient $j$ at the $t$-th visit is calculated by 
\begin{align}
    \mathrm{PRAUC}_j^{(t)} &= \sum_{k=1}^{|\mathcal{M}|}\mathrm{Precision}(k)_j^{(t)}\Delta \mathrm{Recall}(k)_j^{(t)},\notag\\
    \Delta \mathrm{Recall}(k)_j^{(t)} &= \mathrm{Recall}(k)_j^{(t)} - \mathrm{Recall}(k-1)_j^{(t)},
\end{align}
where $k$ is the rank in the sequence of the retrieved drugs, $|\mathcal{M}|$ is the total number of drugs, $\mathrm{Precision}(k)_j^{(t)}$ is the precision at cut-off $k$ in the ordered retrieval list, and $\Delta \mathrm{Recall}(k)_j^{(t)}$ is the change in recall from drug $k-1$ to $k$. The PRAUC for one patient $j$ is by taking the average over her/his visits,
\begin{equation}
    \mathrm{PRAUC}_j = \frac{1}{V_j}\sum_{t=1}^{V_j}\mathrm{PRAUC}_j^{(t)},
\end{equation}
\end{itemize}


% In the experiment, we implement $DDI_j$ from scratch, $Jaccard_j$, $F1_j$ and $PRAUC_j$ are implemented by \textit{scikit-learn} package. Overall, these four metrics will further be averaged over all patients, and we report the final scores in the following sections.

\begin{table*} \label{tb:general}
{\caption{Performance Comparison on
		\textit{MIMIC-III} (ground truth DDI rate is
	0.0808)}
	{\begin{tabular}{l|ccccc} \toprule {\bf Model} & {\bf DDI} & {\bf Jaccard}
			& {\bf F1-score} & {\bf PRAUC} & {\bf Avg. \# of Drugs}\\
			\midrule LR & 0.0829 $\pm$ 0.0009 (0.0) & 0.4865 $\pm$ 0.0021 (0.0) & 0.6434 $\pm$ 0.0019 (0.0) & 0.7509 $\pm$ 0.0018 (3e-11) & 16.1773 $\pm$ 0.0942\\ 
			ECC \cite{read2009classifier} & 0.0846 $\pm$ 0.0018 (0.0) & 0.4996 $\pm$ 0.0049 (5e-10) & 0.6569 $\pm$ 0.0044 (4e-10) & 0.6844 $\pm$ 0.0038 (0.0) & 18.0722 $\pm$ 0.1914\\
				\midrule
			RETAIN \cite{choi2016retain} & 0.0835 $\pm$ 0.0020 (0.0) & 0.4887 $\pm$ 0.0028 (2e-15) & 0.6481 $\pm$ 0.0027 (5e-15) & 0.7556 $\pm$ 0.0033 (2e-06) & 20.4051 $\pm$ 0.2832\\ 
			LEAP \cite{zhang2017leap}  & \underline{0.0731 $\pm$ 0.0008} (0.0) & 0.4521 $\pm$ 0.0024 (0.0) & 0.6138 $\pm$ 0.0026 (0.0) & 0.6549 $\pm$ 0.0033 (0.0) & 18.7138 $\pm$ 0.0666\\ 
			DMNC \cite{le2018dual}  & 0.0842 $\pm$ 0.0011 (0.0) & 0.4864 $\pm$ 0.0025 (2e-16) & 0.6529 $\pm$ 0.0030 (3e-13) & 0.7580 $\pm$ 0.0039 (2e-04) & 20.0000 $\pm$ 0.0000\\ 
			GAMENet \cite{shang2019gamenet}  & 0.0864 $\pm$ 0.0006 (0.0) & \underline{0.5067 $\pm$ 0.0025} (6e-10) & \underline{0.6626 $\pm$ 0.0025} (4e-10) & \underline{0.7631 $\pm$ 0.0030} (0.21) & 27.2145 $\pm$ 0.1141\\ 
			\midrule
			$\method_{L}$ & \textbf{0.058 $\pm$ 0.0004} ($\times$) & 0.5166 $\pm$ 0.0026 (1e-03) & 0.6670 $\pm$ 0.0024 (9e-08) & 0.7632 $\pm$ 0.0026 (0.20) & 18.6663 $\pm$ 0.1417\\ 
			$\method_{G}$ & 0.0606 $\pm$ 0.0007 (7e-06) & 0.4862 $\pm$ 0.0027 (4e-16) & 0.6442 $\pm$ 0.0024 (2e-16) & 0.7423 $\pm$ 0.0029 (4e-13) & 19.0724 $\pm$ 0.0971\\
			\method  & {0.0589 $\pm$ 0.0005} & \textbf{0.5213 $\pm$ 0.0030} & \textbf{0.6768 $\pm$ 0.0027} & \textbf{0.7647 $\pm$ 0.0025} & 19.9178 $\pm$ 0.1604\\
% 			\midrule
% 			$\Delta$ (Improve.) & $\downarrow$ 19.43\% & $\uparrow$ 2.88\% & $\uparrow$ 2.14\% & $\uparrow$ 0.21\% & --\\
			\bottomrule
			\multicolumn{6}{l}{
  \begin{minipage}{17cm}
    \vspace{1mm}
    \noindent~%* $\Delta$ shows the percentage improvements of \method over the best baseline, i.e., $|\method - \mbox{baseline}|$ / baseline. 
    % \fl{can we remove the last row of the table, since the improvement is not significant for Jaccard, F1 and PRAUC.} 
    \\
    ~* We use \underline{underline} to pick the best baseline (excluding our model variants) for each metric and use \textbf{bold} to denote the best method. \\
    ~* We show the $p$-value of student t-test in parenthesis. Smaller $p$-values (usually we hope that $p\leq0.05$) mean that the performance gain over the baseline is more significant. Note that we use ($\times$) for cases where the mean of \method is worse than the baseline.
  \end{minipage}
}
\end{tabular}} \label{tb:comparison}}
\end{table*}

\smallskip
\noindent
\textbf{Implementation Details.} We follow the same setting as \cite{shang2019gamenet} and split  the dataset into training,
validation and test as $\frac23 : \frac16 : \frac16$ randomly.
% \js{60\% DDI rate is way too high. I think the DDI is just a few percents in the real data. We should be lower than that}. 
For embedding tables, $\bm{E}_d$, $\bm{E}_p$, $\bm{E}_a$, we use
$dim=64$ as embedding size. For $\mbox{RNN}_d$ and $\mbox{RNN}_q$, we use gated recurrent unit
(GRU) with $64$ hidden units, since GRU requires fewer parameters but is reported to have
similar power as long short-term memory (LSTM). The dropout rate between two GRU
cells is $0.5$. For MPNN embedding module, the convolution radius $L$ is $2$. For $\mbox{NN}_1(\cdot)$ and $\mbox{MESSAGE}_l(\cdot),~\forall ~l$, we implement as one linear layer
plus basic ReLU activation, for $\mbox{NN}_i(\cdot),~i=2,3,4$, we use linear
functions ($\mbox{NN}_4$ is without bias term), for $\sigma_i(\cdot),~i=1,2,3$, they are all {Sigmoid} activation functions, and we use mean operator for $\mbox{UPDATE}_l,~\forall ~l$. We choose the hyperparameters of \method based on the validation set, where threshold
$\delta$ is $0.5$, the weight $\alpha=0.95$,
$K_p=0.05$, and acceptance rate $\gamma$ is selected $0.06$. Models are implemented in \textit{PyTorch 1.4.0} and parameters are
trained on Adam optimizer \cite{kingma2014adam} with learning rate $2\times 10^{-4}$ for 50 epochs. All the experiments are conducted in
a Linux machine with 30GB memory, 12 CPUs and 1 NVIDIA Tesla V100. We published our data processing scripts and codes in an anonymous repository \footnote{https://github.com/ycqcpsup/SafeDrug}.

In the evaluation, instead of conducting cross-validation, bootstrapping sampling is applied. First, all models are trained on a fixed training set and hyperparameters are selected from a fixed validation set. Then, with replacement, we randomly sample 80\% data points from the test set as on round evaluation. We conduct 10 sampling-evaluation rounds and report the mean and standard deviation values in Table~\ref{tb:comparison}. 


\subsection{AtoQ1: \method Provides More Accurate Recommendations with Lower DDI Rates} \label{sec:general_comparison}

We compared \method with all baseline models and its two model variants. 
We use $\method_{L}$
to denote the model with only bipartite encoder (local, L) and $\method_{G}$ is the
model with only the MPNN encoder (global, G). In implementation, we use $\bm{m}_l^{(t)}$ and $\bm{m}_g^{(t)}$
as the final drug representation for $\method_{L}$ and
$\method_{G}$, respectively, while \method is 
with both modules. 

From Table~\ref{tb:comparison},
it is easy to see sequential based LEAP, DMNC and ECC yield poor results among the baselines, especially for PRAUC. We
therefore conclude that formulating the drug recommendation task as
multi-label prediction might be more straightforward and effective.

Overall, our \method also outperforms the other baselines with significantly lower
DDI rate and better accuracy. In model design, LR and RETAIN do not consider the
DDI information, so they output undesirable DDI rate. Though
considering DDI into the loss function, GAMENet still leads to high DDI. The
reason might be that its recommendations are based on memorizing historical
combinations, however, real medication records usually contain high DDI rate,
e.g., around 8\% in \textit{MIMIC-III}. Also, GAMENet recommends much more drugs than other baselines. Moreover, the performance of two variants, $\method_{L}$ and $\method_{G}$, show that both of the molecular
encoders do help with the prediction, and their integration, \method, performs
even better. In
sum, \method is safe and accurate for recommending drugs

\smallskip
\noindent
\textbf{Significance Test.} 
% \cx{chaoqi, please revise this section. you only need to report how you conduct significant test, and the test results in p values, as well as discuss these results.} 
Next, for each metric, we conduct Student's T-test to determine if there is a significant performance gain over the baseline. 
% The $t$-value is defined as,
% \begin{equation}
%     t = \frac{|{m}_\method - {m}_{baseline}|}{\sqrt{\frac{\sigma^2_\method}{n_1}+\frac{\sigma^2_{baseline}}{n_2}}}
% \end{equation}
% where ${m}$ and $\sigma$ are mean and standard deviation, respectively, $n_1=n_2=10$ are number of sampling rounds. 
In our case, the degree of freedom is $18$. We calculate a $p$-value in terms of two-tailed hypothesis and report in parenthesis
% Specifically, we use $scipy$ package as $p=2\times(1 - scipy.stats.t.cdf(t, df))$.
in Table~\ref{tb:comparison} for each baseline and every metric. Commonly, a $p$-value smaller than 0.05 would be considered as significant. We also use ($\times$) for cases where the result of \method is worse than the baseline.

From the $p$-values, we could conclude that our \method model can beat all compared baselines in almost every metric with $p$=0.001 significance level (smaller is better). For DDI, $\mbox{\method}_{L}$ works slightly better than \method and for PRAUC, our \method beats $\mbox{\method}_{L}$ and GAMENet with about $p$=0.2 significance level. However, \method beats these two baselines in terms of other metrics significantly. Overall, \method outperforms baselines well.


\subsection{AtoQ2: \method Has Less Computational and Space Complexity}
Model complexity of \method and other DL baselines are evaluated in this section. Generally, a model with less computational and space complexity would be favored in deep learning. Also, a light weighted and efficient model would be more understandable and easy to use for healthcare practicers, which is crucial. 

\begin{table}[t!]
{\caption{DL Model Complexity Comparison}
	{\begin{tabular}{l|ccc} \toprule {\bf Model} & {\bf\# of Param.} & {\bf Training Time} & {\bf Inference} \\ \midrule
% 			\midrule LR & $\sim$443,828 & 278.27s (in
% 			Total) & 1.28s \\
			RETAIN & 287,940 &
			36.35s / Epoch & 3.98s
			\\ 
% 			ECC & $\sim$4,438,280 & 21846.16s (in Total) & 101.43s
% 			\\ 
			LEAP  &
			433,286 & 336.14s / Epoch & 32.31s
			\\ DMNC  &
			525,533 & 4697.40s / Epoch & 262.19s
			\\GAMENet  & 449,092 & 162.10s / Epoch & 26.85s \\ \midrule % SafeDrug w/o
			$\method_{L}$  & 299,404 &
			133.43s / Epoch & 9.93s \\ 
			$\method_{G}$  & 324,577 & 129.66s / Epoch & 9.79s \\ % $\beta$-SafeDrug   &
			
			\method  & 325,473 & 138.77s / Epoch & 10.64s\\
			\midrule
			$\Delta$ (improve.) & $\downarrow$ 24.88\% & $\downarrow$ 14.39\% & $\downarrow$ 44.21\%\\
			\bottomrule \multicolumn{4}{l}{
  \begin{minipage}{8cm}
    \vspace{1mm}
    \noindent~* For fair comparisons, we only show improvement over LEAP, DMNC and GAMENet, since RETAIN is not specialized for drug recommendation.
  \end{minipage}
}\\\end{tabular}} \label{tb:comparison2}}
\end{table}

Specifically, we report total number of learnable parameters (excluding hyperparameters), training time and inference time for each method in Table~\ref{tb:comparison2}. 
% Since ECC and LR are not deep learning model, we implement them by {\em scikit-learn} with 500 as maximum iteration. Therefore, their total number of parameters are estimated. We assume that LR learns a separate mapping from the medical codes to individual drugs, so the parameter number is the total number of diagnosis and procedure codes times the size of drug set. ECC uses a 10-member ensemble of classifier chains of independent LR, so its number of parameters is larger than or close to 10 times that of a single LR. The training time of these two methods is the running time of built-in method {\em fit$(\cdot)$}. For other models, 
We report the average running time of each epoch. Note that 
while timing, we kill all other running processes in the machine.
Since RETAIN is not specialized for drug recommendation, improvements in the Table~\ref{tb:comparison2} are over LEAP, DMNC and GAMENet.

Efficiency wise, our model has relatively lower space and time complexity over LEAP, DMNC and GAMENet. Also, it is much more efficient during inference. Leap and DMNC adopt sequential modeling and recommend drug one by one, which is time consuming. GAMENet stores a large memory bank, and thus it requires larger space. By comparison, we conclude that \method is also
efficient and flexible for real deployment.


\subsection{AtoQ3: Study on DDI Controllability} \label{sec:ddi_control}

In clinical decision making, DDIs remain a leading cause of morbidity and
mortality. A DDI-controllable drug recommendation model is therefore important
in practical usage. In this section, we evaluate DDI controllability of our
model. We show that in \method, the average DDI rate
of the output can be controlled by threshold $\gamma$, specifically, $\gamma$
could be interpreted as the acceptance DDI rate.

The ground truth DDI rate in \textit{MIMIC-III} is $0.0808$. We consider that learning based drug recommendation approaches should be able to optimize the final recommendations by processing EHR and drug-drug relation databases, so the output DDI rate is supposed to be lower than human experts'. In this section, we test for a series of targeted DDI $\gamma$
ranging from $0$ to $0.08$. For each $\gamma$, we
train a separate model. We conduct the experiment for 5 times. After convergence, we collect and show the average metrics in
Table~\ref{tb:control}.

\begin{table}[t!] 
\centering 
\caption{Performance under Acceptance DDI Rate $\gamma$}

		\begin{tabular}{c|ccccc} 
		\toprule 
		$\bm{\gamma}$ & {\bf DDI} & {\bf\#
		of Med.} & {\bf Jaccard}  & {\bf F1-score} & {\bf PRAUC} \\ 
		\midrule 
		0.00 & 0.0073  & 13.82 & 0.4198 & 0.5743 & 0.6902 \\ 
		0.01 & 0.0152  & 15.35 & 0.4391 & 0.5924 & 0.6788 \\ 
		0.02 & 0.0254  & 17.64 & 0.4741 & 0.6255 & 0.7196 \\ 
		0.03 & 0.0301  & 18.33 & 0.4959 & 0.6540 & 0.7492 \\ 
		0.04 & 0.0381  & 18.87 & 0.5083 & 0.6651 & 0.7556 \\ 
		0.05 & 0.0479  & 19.08 & 0.5164 & 0.6720 & 0.7604 \\ 
		0.06 & 0.0589  & 19.91 & 0.5213 & 0.6768 & 0.7647 \\ 
		0.07 & 0.0672  & 20.18 & 0.5228 & 0.6776 & 0.7634 \\ 
		0.08 & 0.0722  & 20.75 & 0.5250 & 0.6794 & 0.7691 \\
% 		1.00 &
% 		0.0855  & 23.34 & 0.5305 & 0.6842 & 0.7753 \\
		\bottomrule \end{tabular}
	\label{tb:control}\end{table}



 The result is desirable in our model, DDI
rate of the output is indeed controlled and upper-bounded by $\gamma$ in most
cases, which is consistent with the mechanism of PID controller. It is
interesting that when $\gamma$ becomes larger, more drugs are allowed in
one combination and the accuracy metrics are also improved. However, when
$\gamma$ is too strict ($<0.02$), model performance drops dramatically. In that
case, model will incline to control DDI rather than learn an accurate drug
combination, which could be later complemented by doctors to maintain the efficacy. In sum, with a pre-defined $\gamma$, our model could provide
reliable drug combinations to meet different clinical level of DDI requirements.


\subsection{AtoQ4: Error Analysis} 

Analyzing where and why the model
works or fails is an important step towards deep understandings. In this
section, we perform model analysis on DDI rates and number of medications/drugs in
terms of the test data. Our conclusion is that \method performs better in the scenario when a visit has lower actual DDI rate or involves more medications.

Formally, we  evaluate on the following two
scenarios based on the whole test set: (i) we use ground truth DDI ($0.00\sim0.20$) as threshold and
remove those test points with lower DDI rates; (ii) use \# of medications
($0\sim30$) as threshold and remove those test points with smaller drug
set. For each test scenario, we calculate four evaluation metrics plus the avg. \# of med. and draw the trends in Figure~\ref{fig:analysis}. When two threshold equals to $0$, it should show a similar \method result as Table~\ref{tb:comparison}.

\begin{figure*}[t!] \centering
	\includegraphics[width=6.8in]{figure/ablation_safedrug.pdf}
	\caption{Performance Analysis with respect to DDI and \# of Med. in Various
		Test Scenarios 
% 		\js{No sure what the message is. We should move this figure to supplement.}
		} \label{fig:analysis} \end{figure*}
		
When the DDI threshold increases or the
medication threshold decreases, the overall performance will drop. The reason
might be that on the one hand, if the ground truth DDI is high, our model tends
to recommend fewer drugs for a lower DDI combination, thus leading to a
sacrifice on the accuracy; on the other hand, when formulating the task as a
multi-label prediction problem, a smaller ``\# of med" threshold means less data and more noise, which undermines the model.

\subsection{AtoQ5: Effectiveness of Mask Matrix to avoid Interacted Drugs} \label{sec:case1}
		

In this section, we hope to interpret the benefit of bipartite mask $\bm{H}$. For preparation, we load the pre-trained \method model (from Section~\ref{sec:general_comparison}) and extract the parameter matrix, $\mbox{MASK}(\bm{W}_4,\bm{H})$, denoted by $\bm{W}\in\mathbb{R}^{|\mathcal{S}|\times|\mathcal{M}|}$. We inspect the {\em learned weights} correspond to interacted drug pairs. From experiments, we will see the interacted drugs have negative-correlated weights, which means {\em they are less likely to be co-prescribed by our model.} Below are more details.
 
 
 
\smallskip
\noindent
\textbf{Basics of $~\bm{W}$.} On average, when constructing the bipartite structure $\bm{H}$ by fragmentation, each drug (right cells in the bipartite architecture in Figure~\ref{fig:framework}) is connected to 6.84 out of $|\mathcal{S}|=$ 491 functional substructures (left cells) and conversely, each substructure is connected to 1.82 out of $|\mathcal{M}|=$ 131 drugs. Thus, $\bm{W}$ is a sparse matrix. Each element of $\bm{W}$, for example, $\bm{W}_{ij}$ quantifies the weight relation between a  substructure $i$ and a particular drug $j$.



\smallskip
\noindent
\textbf{Evaluation Procedure.} For drug $j$, its functional weight representation is the $j$-th column of the weight matrix, $\bm{W}_{:,j}$, a {\em sparse} real-valued vectors of size, $|\mathcal{S}|$, where $\mathcal{S}$ is the overall substructure set.
To evaluate the efficacy of DDI reduction, we hope that for a pair of interacted drugs, e.g., $i$ and $j$, the cosine similarity of their weight representation is negative, i.e., 
\begin{equation}
    cos(\bm{W}_{:,i}, \bm{W}_{:,j}) = \frac{\bm{W}_{:,i}\cdot\bm{W}_{:,j}}{\|\bm{W}_{:,i}\|\cdot\|\bm{W}_{:,j}\|}<0,
\end{equation} 
% {\em Examples.} We first randomly select $5$ interacted drug pairs and $5$ non-interacted drugs pairs and illustrate their weight correlations in Table~\ref{tb:example}. Roughly, we can observe that the interacted drugs tend to have negative correlation and those non-interacted drugs will have arbitrary weight correlation. To quantitatively evaluate on the whole dataset, we design the following metrics.
% \begin{table}[!t] \centering \caption{5 Interacted and 5 Non-interacted Examples (drugs are coded by ATC Third Level)} 
% 		\begin{tabular}{cc|cc} 
% 		\toprule 
%         drug $i$ & drug $j$ & interaction & $\sigma(\bm{W}_{:,i})^\top\sigma(\bm{W}_{:, j})$ \\
%         \midrule
%         $N04B$ & $C09A$ & $\surd$ & -0.0513 \\
%         $M04A$ & $N05C$ & $\surd$ & 0.0000 \\
%         $G04B$ & $C09C$ & $\surd$ & -0.0631 \\
%         $B01A$ & $N04B$ & $\surd$ & -0.0082 \\
%         $B01A$ & $R05D$ & $\surd$ & -0.0330 \\
%         $G04C$ & $C01B$ & $\times$ & 0.0468 \\
%         $D05A$ & $D06A$ & $\times$ & 0.0000 \\
%         $B01A$ & $N07B$ & $\times$ & -0.0232 \\
%         $G03A$ & $L04A$ & $\times$ & 0.0000 \\
%         $A04A$ & $G04B$ & $\times$ & 0.0201 \\
% 		\bottomrule 
% 		\multicolumn{4}{l}{
%           \begin{minipage}{7cm}
%             \vspace{1mm}
%             \noindent~* We can observe that the interacted drugs tend to have {\em negative correlation}, and those non-interacted drug pairs have arbitrary weight correlation.
%           \end{minipage}
%         }
% 		\end{tabular}
% 	\label{tb:example}\end{table}
which prevents their co-prescription. For {\em all  pairs of interacted drugs}, we design the average cosine similarity, $Cos_{interacted}$, 
\begin{equation}
    Cos_{interacted} = \frac{\sum_{i,j:~\bm{D}_{ij}=1} cos(\bm{W}_{:,i}, \bm{W}_{:,j})}{\sum_{i,j:~\bm{D}_{ij}=1}1},
\end{equation}
where $\bm{D}$ is the DDI matrix. And for {\em all possible drug pairs}, we design the average cosine similarity, $Cos_{all}$,
\begin{equation}
    Cos_{all} = \frac{\sum_{i,j:~i\neq j} cos(\bm{W}_{:,i}, \bm{W}_{:,j})}{\sum_{i,j:~i\neq j}1}.
\end{equation}
Following the intuition, we hope that $Cos_{interacted}$ could be much smaller than $Cos_{all}$. To conduct ablation study for mask $\bm{H}$, we remove it and run the experiment again with the settings reported in Section~\ref{sec:setting}. We show the $Cos_{interacted}$ and $Cos_{all}$ as well as the output DDI of two cases in Table~\ref{tb:competing}. 
		
\begin{table}[h!] \centering \caption{$Cos_{interacted}$, $Cos_{all}$ and output DDI vs Mask $\bm{H}$} 
		\begin{tabular}{c|ccc} 
		\toprule 
		with mask $\bm{H}$ & $Cos_{interacted}$ & $Cos_{all}$ & output DDI\\ 
		\midrule 
% 		0.00 / 0.06 & Yes & -0.0051 / -0.0006 & 0.0018 / 0.0022 \\
% 		0.00 & Yes & -0.0051 & 0.0018 & 0.0093\\
% 		0.06 & Yes & -0.0006 & 0.0022 & 0.0515\\
% 		0.00  & No & 0.3403 & 0.1202 &  0.0117\\
% 		0.06 & No & 9.9766 & 1.5741 & 0.0588\\
		
		Yes & -0.0030 & 0.0021 & 0.0589 \\
		No & 0.0036 & 0.0017 & 0.0652\\
		\bottomrule 
		\multicolumn{4}{c}{
          \begin{minipage}{7cm}
            \vspace{1mm}
            \noindent~* With mask $\bm{H}$, $Cos_{interacted}<0<Cos_{all}$ is observed, which indicates that the interacted drugs are less likely to be co-prescribed. Without mask $\bm{H}$, the model cannot identify and prevent interacted drugs. In practice, the case without mask $H$ may also have low DDI because of our proposed controllable loss function.
          \end{minipage}
        }
        \end{tabular}
	\label{tb:competing}\end{table}
	
\smallskip
\noindent
\textbf{Results and Interpretation.} As is mentioned, $\bm{W}$ is sparse, so the calculated cosine similarities all have low magnitudes, and it does not necessarily mean that the correlation is not significant. It is interesting that \method with mask $\bm{H}$ have $Cos_{interacted}<0<Cos_{all}$, which means the mask does enable the model to send negatively-correlated signals for interacted drugs, so that the output DDIs decrease in the final combination. We  observe that the model without $\bm{H}$ (i.e., $\mbox{NN}_4$ is a fully connect network) 
% could also provide desirable DDI rate under our PID loss controller, however, it 
cannot distinguish interacted drug pairs, and the correlation value $Cos_{interacted}$ of the interacted drugs is even larger than $Cos_{all}$ of all drug pairs, which is undesirable and counter-intuitive. The reason why its DDI value is also lower than other baselines is due to the DDI loss and our proposed controllable loss function.
% We conclude that in this problem, 
% % a direct fully connect network (FCN) is more of a black-box, 
% our bipartite structure design is interpretable and effective.

% \subsection{Case Study2: Sanity Check on the Learned Diagnosis or Procedure Embeddings.}

% \begin{figure}[!htbp] \centering
% 	\includegraphics[width=3.4 in]{figure/Umap-projection.pdf}
% 	\caption{UMAP Projection of Learned Diagnosis and Procedure Embeddings. The color is given by 1-dimension PCA projection of diagnosis-drug co-occurance matrix (for the left figure) and procedure-drug co-occurance matrix (for the right figure) from the training set.} \label{fig:umap} \end{figure}

% In this section, we check whether the learned patient functional vector $\bm{m}^{(t)}_f$ accords with groud-truth drug functionalities. Specifically, we randomly selected 10 patients and extract the most salient substructures, which corresponds to top-3 largest elements in $\bm{m}^{(t)}_f$. Then we check whether these three substructures exist in real drug combination $\bm{m}^{(t)}$. Note that we only evaluate their last observed visit. The result is shown in Table~\ref{}....
		

% In this section, we inspect the medication correlation within two consecutive
% visits and tempt a even better model on top of \textit{SafeDrug}. For the drug
% recommendation task, the key is to learn a mapping from patient health history
% to medication representation. However, a closely-related and more realistic
% task is to learn drug replacement from the last visit. Our motivations stem
% from the fact that within two consecutive clinical visits, the medications are
% heavily overlapped.

% \subsubsection{Observation.} For each patient $T$, we first collect their
% medication sets during each visit as a temporal sequence
% $M_T=[m_T^1,\dots,m_T^{V(T)}]$ from \textit{MIMIC-III} dataset. We calculate
% the average Jaccard correlation between two consecutive visits for each $M_T$
% and then take further average over all patients, i.e., all $M_T$. We obtain
% 0.4512, which is the correlation value between two consecutive visits for the
% \textit{MIMIC-III} dataset. Next, we concatenate the medication sequences of
% all the patients as a compound sequence $M$,
% \begin{align}
%     M &= M_1~\#~M_2~\#~\dots \notag\\
%     &= [m_1^1,\dots,m_1^{V(1)},m_2^1,\dots,m_2^{V(2)},\dots] \notag
% \end{align}
% Then, we randomly shuffle $M$, calculate the Jaccard correlation between two
% consecutive records and then take the average. The shuffle-and-calculate
% process takes 2000 times, and the distribution of the average value for each
% trial is shown in Figure~\ref{fig:dist} with the mean value at around 0.3050.
% This mean value roughly indicates the random Jaccard correlation over the
% dataset. By comparison, we can clearly conclude that in average, the
% medication sets during a patient's two consecutive have strong
% correlations/overlaps.

% We therefore adopt the concept of drug replacement and learn to replace (add
% and delete) some of the drugs in the last visit as the recommended combination
% for the current visit. To fulfill this, we propose residual learning based
% \textit{Res-SafeDrug}, which shares the same \textit{SafeDrug} architecture
% but with different training and inference procedures.

% \subsubsection{Training.} Let $h^t$ denote the patient health representation
% at $t$-th visit, and $y^{t}$ as the target medication set. For
% \textit{SafeDrug} model, we train on each pair of $(h^t, y^t)$. For the
% \textit{Res-SafeDrug} model, we train on two consecutive visits at once (as
% data augmentation): (i) feed $h^{t-1}$ to the embedding modules and get
% $\hat{y}^{t-1}$; (ii) feed the residual health representation $h^{t} -
% h^{t-1}$ to the embedding modules and get $\hat{r}^t$; (iii) regard $\hat{y}^t
% = \hat{y}^{t-1} + \hat{r}^{t}$. Then the loss is calculated by comparing 
% $\hat{y}^{t-1}$ with $y^{t-1}$ and $\hat{y}^t$ with $y^{t}$. From a
% higher-level, the \textit{SafeDrug} model can only read the patient health
% representation, but the \textit{Res-SafeDrug} model is able to read the
% residual health representations, which is an update/residual.

% \begin{figure}[tbp!]
% 	\centering
% 	\vspace{-4mm}
% 	\includegraphics[width=3.2in]{figure/dist.pdf}
% 	\vspace{-3mm}
% 	\caption{Distribution of Correlation in Random Order}
% 	\label{fig:dist}
% \end{figure}

% \subsubsection{Inference.} The final drug recommendation is a residual update
% on the basis of the last visit, which elaborates the concept of drug
% replacement. In \textit{SafeDrug}, we set medication threshold $\delta=0.5$ on
% the final representation $\hat{m}^t$, when $\hat{m}_i^t>\delta$,  then drug
% $i$ will be picked. In \textit{Res-SafeDrug}, we have $\delta_1 = 0.9$ as the
% “adding” threshold, if any $\hat{m}_i^t>\delta_1$, we add the drug to the
% base; similarly, we have $\delta_2 = 0.1$ as the “deleting” threshold, if any
% any $\hat{m}_i^t<\delta_2$, we delete drug $i$ from the base, which leading to
% the new drug combination for the current visit. It is interesting that when
% $\delta_1 = \delta_2 = \delta$, then \textit{Res-SafeDrug} reduces to
% \textit{SafeDrug}.

% \subsubsection{Analysis and Discussion.} The \textit{Res-SafeDrug} model is
% evaluated under the same setting in Table~\ref{tb:res-result} (PRAUC is not
% applicable for \textit{Res-SafeDrug}). We can observe that
% \textit{Res-SafeDrug} has slightly higher DDI rate (since it is built on
% \textit{SafeDrug} and not directly trained on DDI loss), fewer number of
% medications, and significantly higher Jaccard and F1. Clearly,
% \textit{Res-SafeDrug} is better than \textit{SafeDrug}. We think the concept
% of residual learning opens a new option for safe drug recommendation task. In
% the future, we shall explore how to directly include the DDI loss into
% residual learning.

% \begin{table}[tbp!] \small
%     \centering
%     \caption{Performance Comparison}
%     \begin{tabular}{l|ccccc}
%     \toprule
%             & DDI & \# of Med. & Jaccard  & F1 \\
%          \midrule
%          SafeDrug & 0.0515 & 22.67 & 0.5243 & 0.6750 \\
%          Res-SafeDrug & 0.0539 & 21.18 & 0.5407 & 0.6938 \\
%          \bottomrule
%     \end{tabular}
%     \label{tb:res-result}
%     \vspace{-1mm}
% \end{table}

% \begin{table*}[htbp!] \small
%     \centering
%     \vspace{-4mm}
%     \caption{Performance of SafeDrug / Res-SafeDrug under Different Target DDI
% Rate (no embedding).}
%     \begin{tabular}{c|ccccc}
%     \toprule
%       $\gamma$ & DDI & \# of Med. & Jaccard  & F1 \\
%          \midrule
%          0.00 & 0.0071 / 0.0116  & 17.05 / 16.47 & 0.4648 / 0.4816 & 0.6262 /
% 0.6422 \\
%          0.01 & 0.0117 / 0.0153  & 19.14 / 18.42 & 0.4802 / 0.4927 & 0.6404 /
% 0.6522 \\
%          0.02 & 0.0213 / 0.0271  & 19.73 / 18.93 & 0.4998 / 0.5152 & 0.6579 /
% 0.6718 \\
%          0.03 & 0.0311 / 0.0387  & 20.58 / 19.71 & 0.5115 / 0.5304 & 0.6681 /
% 0.6851 \\
%          0.04 & 0.0346 / 0.0436  & 20.73 / 19.95 & 0.5118 / 0.5346 & 0.6684 /
% 0.6887 \\
%          0.05 & 0.0429 / 0.0486  & 21.41 / 20.40 & 0.5178 / 0.5386 & 0.6736 /
% 0.6921\\
%          0.06 & 0.0534 / 0.0561  & 22.51 / 21.27 & 0.5208 / 0.5430 & 0.6761 /
% 0.6956  \\
%          0.07 & 0.0576 / 0.0596  & 23.02 / 21.60 & 0.5225 / 0.5440 & 0.6776 /
% 0.6966 \\
%          0.08 & 0.6059 / 0.0667  & 23.63 / 22.06 & 0.5231 / 0.5451 & 0.6786 /
% 0.6995 \\
%          \bottomrule
%     \end{tabular}
%     \vspace{-1mm}
% \end{table*}



==> cover_letter/introduction.tex <==
\section{Introduction} 
% In modern predictive healthcare, various deep learning models
% have been developed to assist the doctors for important clinical decisions such as diagnosis \cite{choi2016doctor,choi2017using,xiao2018opportunities,sendak2020human,li2020behrt}
% and treatment \cite{wang2017safe,shang2019gamenet,shang2019pre,wang2020adversarial},
% thanks to the increasing availability of large longitudinal electrical health records (EHR). In the area of
% drug recommendation, traditional rule-based methods
% \cite{almirall2012designing,chen2016physician}, defined by clinical guidelines or
% medication instructions, are gradually substituted or improved by deep neural
% networks especially in complex comorbidity situations~\cite{zhang2017leap,shang2019gamenet,wang2019order,shang2019pre}. 

Today abundant health data such as longitudinal electronic health records (EHR) and massive biomedical data available on the web enable researchers and doctors to build better predictive  models for
clinical decision making, such as diagnosis \cite{choi2016doctor,choi2017using,xiao2018opportunities,sendak2020human,li2020behrt}
and treatment \cite{wang2017safe,shang2019gamenet,shang2019pre,wang2020adversarial}. Among others, recommending effective  and safe medication combination is an important task especially for helping patients with complex health conditions~\cite{wang2017safe,shang2019gamenet,shang2019pre,wang2020adversarial}. The primary goal of recommending medication combination is to customize a safe combination of drugs for a particular patient based on health conditions of the patient. 
% Different from common supervised classification
% tasks, where the model targets on a single label, the problem of drug
% recommendation can be viewed as a multi-label  classification
% \cite{zhang2017leap,shang2019gamenet}, where the model predicts a set of drugs per recommendation. 
Over the years, a series of deep learning methods have been designed for medication recommendation. Earlier ones are \textit{instance-based} which perform recommendation based only on the current hospital visit ~\cite{zhang2017leap,wang2017safe}.
As a result, a patient with newly diagnosed hypertension will likely be treated the same as another patient who has suffered chronic uncontrolled hypertension.  Such a limitation affects safety and utility of the recommendations. To overcome this issue, \textit{Longitudinal} methods such as ~\cite{choi2016retain,lipton2015learning,le2018dual,shang2019gamenet,wang2019order} are proposed. They leverage the temporal dependencies within longitudinal patient history to provide more personalized medication recommendation. However, they still suffer from the following limitations.


\begin{itemize}[leftmargin=*]
    \item {\bf Inadequate Medication Encoding.}  Existing works  \cite{wang2017safe,wang2018supervised,shang2019gamenet,wang2019order}  often simply represent medications using one-hot encoding where each drug  is considered a (binary) unit, ignoring that drugs in their meaningful molecular graph representation which encodes important  drug properties. For example, drugs' molecule information such as structures and substructures are highly related to their efficacy and safety profiles. Such knowledge are accumulated on the web~\footnote{For example, molecule data can be found on \url{drugbank.com}} and can be useful for improving accuracy and safety in medication recommendation. 


\item {\bf Implicit and Non-controllable DDI Modeling.} Some existing works model drug-drug interactions (DDI) via soft or indirect constraints. For example, in ~\cite{wang2017safe,mao2019medgcn} complex medical knowledge graphs (KG) are leveraged to capture DDI relations, while DDI relations are implicitly modeled and only count toward a small fraction of all complex entity-relation-entity triplets in the KGs. In addition, in \cite{zhang2017leap} the authors employ reinforcement fine-tuning to prevent DDIs in the final recommendations, however, this post-processing approach will potentially break the integrity and thus needs accuracy trade-off of the recommendations, which is a sub-optimal solution. These implicit handling of DDIs results in non-controllable rates in the final recommendation or sub-optimal recommendation accuracy.
\end{itemize}

To address these limitations, we propose a DDI-controllable
drug recommendation model, named \method, to leverage drugs' molecule structures and to model DDIs explicitly. \method takes both patient EHR and drug molecule data  as input. It firstly learns {\em patient representation} and feed  them into two  molecular graph encoders, i.e., a global message passing neural network (MPNN) module and a bipartite learning module. The MPNN encoder outputs a {\em global drug vector} by matching the learned patient representation to each of the drug global representation, generated by message passing across the whole molecule graphs. In parallel, the bipartite encoder also feeds on the same patient representation and generates a {\em local drug vector}, which encodes drug molecular local functionalities with {\it an effective masked neural network}. The final output is obtained by element-wisely integration of the global and local drug vectors. They are then trained with a controllable loss function design to effectively control DDI level in the recommended drug combinations.

\smallskip
\noindent\textbf{Contribution}. To summarize, \method is enabled by the following technical contributions:
\begin{itemize}[leftmargin=*]
\item \textbf{Dual Molecular Encoders to Capture Global and Local Molecule Patterns.} \method uses dual molecule encoders to capture the global pharmacological properties~\cite{brown1868connection} and the local sub-structural patterns of a drug~\cite{huang2020caster}. Globally, an  MPNN encoder is constructed to pass molecular information message for the whole drug  layer by layer, where drug connectivity information is well captured in multiple hops. Locally, a bipartite encoder segments drug molecules into substructures, each possibly associated with small functional groups. The patient to drug mapping and DDI reduction are therefore obtained from the substructure-level with an effective masked neural network.
\item \textbf{DDI Controllable Loss Function.} Inspired by  proportional-integral-derivative (PID) controller \cite{an2018pid,aastrom1995pid}, we design a new technique to adaptively combine supervised loss and unsupervised DDI constraints with considerable flexibility. During the training, the negative DDI signal would be emphasized and backpropagated if the DDI rate of individual samples is above certain threshold/target. In the experiment, the adaptive gradient descending manner is able to balance the model accuracy and final DDI level. With a preset DDI target, \method model can provide reliable drug combinations to meet different levels of DDI requirements.
\end{itemize}
We follow previous works~\cite{zhang2017leap,shang2019gamenet,le2018dual} and evaluate \method on a benchmark medication recommendation  dataset extracted from the
\textit{MIMIC-III} database \cite{johnson2016mimic}. \method outperforms the best baselines  by 19.43\% relative improvement in DDI reduction, 2.88\% in Jaccard similarity and 2.14\% in F1 measure. Besides, \method requires much fewer parameters than previous deep learning based drug recommendation approaches with 14\% reduction in training time and around $2\times$ speed-up during inference. For the safety purpose, we also evaluate the model in terms of DDI controllability. The results show that \method is flexible and can be tailored to meet different levels of DDI requirements. 



==> cover_letter/method.tex <==
\section{The \method Model} \label{sec:method}

\begin{figure*}[htbp!] \centering
	\includegraphics[width=6.9in]{figure/safedrug_model2.png} \caption{The \method
		Model. We first encode diagnosis and procedure sequences by {RNN}s to generate a patient health representation, $\bm{h}^{(t)}$; this representation then passes through dual molecular graph encoders (an MPNN embedding module and a bipartite embedding module) for global and local molecular structural embeddings, $\bm{m}_g^{(t)}$ and $\bm{m}_l^{(t)}$; two embedding vectors are finally combined and thresholded to obtain the recommended drug combination, $\hat{\bm{m}}^{(t)}$.
% 		\js{More description of the pipeline should be added as part of the caption.}
		} \label{fig:framework} \end{figure*}

As illustrated in Figure~\ref{fig:framework}, \method comprises of four components: (1)  a {\bf longitudinal patient representation module} that learns patient representation from their EHR data; (2)  a {\bf global message passing neural network (MPNN) encoder} that takes patient representation as input and outputs a global drug vector with each entry quantifying the similarity between the 
patient representation and each of the drug representations; (3) in parallel, a {\bf bipartite encoder} also takes the same patient representation and outputs a local drug vector, which encodes drugs' molecular substructural functionalities; (4) finally, the global and local drug representation vectors are element-wise combined in {\bf  medication representation module}, where the final drug output is obtained from element-wise thresholding.

\subsection{Longitudinal Patient Representation} During a clinical visit, doctors
would first \textit{diagnose} for the diseases and then therapeutic
\textit{procedures} are applied. Based on these two steps, the doctors are
ready to prescribe drugs. In this work, the patient's health condition is also extracted on the basis of both \textit{diagnosis} and \textit{procedure} information.

\smallskip
\noindent
\textbf{Diagnosis Embedding.} To fully utilize rich diagnosis information, we design an embedding table,
$\bm{E}_d\in \mathbb{R}^{|\mathcal{D}|\times dim}$, where each row stores the embedding vector
for a particular diagnosis and $dim$ is
the dimension of the embedding space. Given a multi-hot diagnosis vector $\bm{d}^{(t)}\in
\{0,1\}^{|\mathcal{D}|}$, we project the corresponding diagnosis codes into the embedding space by vector-matrix dot product, \begin{equation}\label{eq:diag-emb} \bm{d}^{(t)}_e = \bm{d}^{(t)} \cdot \bm{E}_d.
\end{equation}
During the training, $\bm{E}_d$ is learnable and shared between each visit and every patient. 

\smallskip
\noindent
\textbf{Procedure Embedding.} Similarly, a shared procedure table
$\bm{E}_p\in \mathbb{R}^{|\mathcal{P}|\times dim}$ is also designed to encode the
associated procedure vector $\bm{p}^{(t)}$ (also a multi-hot vector), \begin{equation} \label{eq:prod-emb}
\bm{p}^{(t)}_e = \bm{p}^{(t)} \cdot \bm{E}_p. \end{equation}
Two {\em embedding vectors}, $\bm{d}^{(t)}_e,\bm{p}^{(t)}_e\in\mathbb{R}^{dim}$, encode the patient's current health condition. In fact, a health snapshot might be insufficient for treatment decision. For example, it is
inappropriate to prescribe the same medicine for one patient with a newly
diagnosed hypertension and another patient who has chronic hypertension for more
than two years. 
Here we use RNN models to model  dynamic patient history. Specifically, we use two separate {RNN}s to obtain the {\em hidden diagnosis and procedure vectors}, $\bm{d}^{(t)}_h$ and $\bm{p}^{(t)}_h$, in case that
one of the sequences might be inaccessible in practice,
\begin{align} \bm{d}^{(t)}_h &=
\mbox{RNN}_d~(\bm{d}^{(t)}_e,\bm{d}^{(t-1)}_h)
= \mbox{RNN}_d~(\bm{d}^{(t)}_e,\bm{d}^{(t-1)}_e,\dots,\bm{d}^{(1)}_e), \label{eq:hidden-diag}\\
\bm{p}^{(t)}_h &=
\mbox{RNN}_p~(\bm{p}^{(t)}_e,\bm{p}^{(t-1)}_h)
= \mbox{RNN}_p~(\bm{p}^{(t)}_e,\bm{p}^{(t-1)}_e,\dots,\bm{p}^{(1)}_e), \label{eq:hidden-prod}
\end{align} 
where $\bm{d}^{(t)}_h,\bm{p}^{(t)}_h\in\mathbb{R}^{dim}$. And $\bm{d}^{(0)}_h$ and $\bm{p}^{(0)}_h$ are all-zero vectors.

\smallskip
\noindent
\textbf{Patient Representation.} 
We then concatenate the diagnosis embedding $\bm{d}^{(t)}_h$ and  procedure embedding $\bm{p}^{(t)}_h$  into a more compact {\em patient representation} $\bm{h}^{(t)}$. We follow a common and effective
approach  to first \textit{concatenate} two vectors as a double-long vector,
and then apply a feed-forward neural network, $\mbox{NN}_1(\cdot): \mathbb{R}^{2dim}
\mapsto \mathbb{R}^{dim}$,
($\bm{W}_1$ is the parameter, and $\#$ is the concatenation operation), \begin{equation}\label{eq:patient_rep} \bm{h}^{(t)}
= \mbox{NN}_1([\bm{d}^{(t)}_h ~ \# ~\bm{p}^{(t)}_h]; \bm{W}_1). \end{equation}

So far, we obtain an overall patient representation
$\bm{h}^{(t)}\in\mathbb{R}^{dim}$. Next, we start from $\bm{h}^{(t)}$ and generate a safe drug recommendation by comprehensively modeling the drug molecule databases. 

\subsection{Dual Molecular Graph Encoders} 

To investigate drug properties and their dependencies, we exploit the
global molecule connectivity features and the local molecule functionalities. In the following sections, we introduce two novel molecular graph encoders, in parallel, to comprehensively encode
the drug molecules.


\subsection*{(I) Global MPNN Encoder} 
The chemical structure of a
drug is proven as a powerful indicator of the property
\cite{brown1868connection,yang2019analyzing}. Here, we design a message passing neural network (MPNN)
% \js{specify the full name of MPNN once here} 
operator with learnable fingerprints. The MPNN encoder aims at convolving atom information across drug molecule graphs and pooling into informative vector representations.


To begin with, we collect a set of all appeared atoms, $\mathcal{C}=\{a_i\}$, and design a learnable atom
embedding table, $\bm{E}_a\in\mathbb{R}^{|\mathcal{C}|\times dim}$, where each row
looks up the initial embedding/fingerprint for a particular atom. Our design with MPNN model is very different from previous works \cite{coley2017convolutional,yang2019analyzing}, which mostly use atom descriptors, e.g., atom mass and chirality, as the initial features. However, for molecule structure modeling, atom-atom connectivity is more important than individual atoms, and the descriptor features are likely to introduce more noise.

Given a
drug molecule graph (atoms $a_0, \dots, a_n$ as the vertices and atom-atom bonds as
edges) with adjacency matrix $\bm{A}$ and the initial atom fingerprints from $\bm{E}_a$,
i.e., $\{\bm{y}_0^{(0)},\bm{y}_1^{(0)},\dots, \bm{y}_n^{(0)} \}$, we formulate the layer-wise message passing over the graph as,
\begin{align}
\bm{z}_i^{(l+1)} &= \sum_{j:~\bm{A}_{ij}=1}\mbox{MESSAGE}_l~(\bm{y}_i^{(l)}, \bm{y}_j^{(l)}; \bm{W}^{(l)})
\label{eq:z_i}\\ %     y_j^{(i+1)} &= \frac{z_j^{(i)}+\sum_{A_{jk}=1}
% z_k^{(i)}}{1 +\sum_{A_{jk}=1}1 },~j=0,\dots,n
\bm{y}_i^{(l+1)} &= \mbox{UPDATE}_l~(\bm{y}_i^{(l)}, \bm{z}_i^{(l+1)}),~i=0,\dots,n \label{eq:y_i}\end{align} 
where $l$ is the layer index, $\bm{z}_i^{(l+1)}$ is the encoded messages from the neighbors of atom $i$ at the $l$-th iteration, $\bm{y}_i^{(l+1)}$ is the hidden state of atom $i$. During message passing, $\bm{z}_i^{(l+1)}$ and $\bm{y}_i^{(l+1)}$ with each vertex atom $i$ are updated using {\em message function}, $\mbox{MESSAGE}_l(\cdot)$, and vertex {\em update function}, $\mbox{UPDATE}_l(\cdot)$, and $\bm{W}^{(l)}$ is the layer-wise parameter matrix. After applying message passing for $L$ layers, the global representation of a drug molecule is pooled
by a {\em readout function}, which (in this paper) calculates the average of all atom fingerprints, \begin{equation} \label{eq:y} \bm{y} = \mbox{READOUT}~(\{\bm{y}_i^{(L)}\mid i=0,\dots,n\}). \vspace{1mm}\end{equation} 
For each candidate drug (there are $|\mathcal{M}|$
different drugs in total), we apply the same MPNN encoder with shared parameters. We therefore
obtain a drug memory  $\bm{E}_g\in\mathbb{R}^{|\mathcal{M}|\times dim}$,
where each row is the global MPNN representation of a drug.




\smallskip
\noindent
\textbf{Patient-to-drug Matching.} When treating patient
representation $\bm{h}^{(t)}$ as a query, we aim at searching the most {\em relevant} drugs
from the memory $\bm{E}_g$. The health-to-drug matching score is calculated by
the dot product of the MPNN representation and the patient representation $\bm{h}^{(t)}$. For all drugs, we operate each row of $\bm{E}_g$ with $\bm{h}^{(t)}$, followed by an activation function $\sigma_1(\cdot)$,
% \js{Use $\sigma()$ for sigmoid function} 
% with another
% neural network $\mbox{NN}_2(\cdot)$ for further drug representation scoring,
\begin{align} \label{eq:relevant}\bm{m}_r^{(t)} &= \sigma_1~(\bm{E}_g\cdot \bm{h}^{(t)} ).\end{align}
Every element of $\bm{m}_r^{(t)}$ stores a matching score for one drug. Similar to \cite{vaswani2017attention}, the matching score is further parametrized  by a feed-forward neural network, $\mbox{NN}_2(\cdot): \mathbb{R}^{dim}
\mapsto \mathbb{R}^{dim}$, followed by layer-normalization (LN) step with residual connection,
\begin{align}\label{eq:global} \bm{m}_g^{(t)} &= \mbox{LN}~(\bm{m}_r^{(t)}+\mbox{NN}_2~(\bm{m}_r^{(t)};\bm{W}_2)).\end{align}
% \js{Where are the details of NN2?}



\subsection*{(II) Local Bipartite Encoder} 

Molecules with similar
structures shall be mapped into nearby space using MPNN encoder.  However, 
a pair of drugs that have significant overlap on structure domain might behave
differently in terms of DDI interaction or other functional activities
\cite{silverman2014organic,ryu2018deep}. 
%For example, dimethyltryptamine (DMT) and serotonin only differ in a hydroxyl group. However, the former is used for temporary relief of nervousness while the latter works as an agonist or an antagonist. 
In fact, the functionality of a drug is better reflected by molecule
substructures, which are defined as a set of connected atoms that may have associated functional groups. This section focuses on the substructure composition of molecules and builds a  substructure-to-drug bipartite architecture for capturing drug local functionality and their dependencies.



\smallskip
\noindent
\textbf{Molecule Segmentation.} 
To capture the relations between drug molecules and its substructures, we first adopt the well-known molecule segmentation method, breaking of retrosynthetically interesting chemical substructures (BRICS) \cite{degen2008art}. During the fragmentation, some pharmacophore of drugs might be broken. However, BRICS still preserves most critical drug functional groups and more crucial bonds than its substitutes \cite{liu2017break}. Our \method can easily support other  segmentation methods such as RECAP \cite{lewell1998recap}.%, detailed discussions are beyond the scope of this paper.
% \js{what are the other methods? can we cite some?} 
  After the segmentation, each molecule is decomposed
into a set of chemical substructures. 
In this setting, a pair of drugs could intersect on a mutual set of substructures. We denote the overall substructure set as $\mathcal{S}$. Based on the many-to-many relations, it is ready to construct a
bipartite architecture (in Figure~\ref{fig:framework} within bipartite encoder, substructure set is on the left and the drug set  on the right), represented by a {\it mask matrix} $\bm{H}\in \{0,1\}^{|\mathcal{S}|\times |\mathcal{M}|} $: $\bm{H}_{ij}=1$ indicates that drug $j$ contains  substructure $i$, otherwise, $\bm{H}_{ij}=0$.
% \js{describe the size of $H$ using bold font. Adding a figure of the architecture will be helpful.}


\smallskip
\noindent
\textbf{Bipartite Learning.} 
% \js{This subsection is unclear. We need to motivate this architecture and then describe this formally. Right now it is vague w/o motivation why this mask architecture is better. In fact, we should compare w/ one w/o  }
We hope that $\bm{H}$ can help to derive a drug representation on its functionality information, given the input, $\bm{h}^{(t)}$. To do so, we first apply a feed-forward neural network,
$\mbox{NN}_3(\cdot): \mathbb{R}^{dim}
\mapsto \mathbb{R}^{|\mathcal{S}|}$, for dimensionality transformation, followed by an activation function, $\sigma_2(\cdot)$. In fact, $\mbox{NN}_3(\cdot)$ transforms the patient representation $\bm{h}^{(t)}$ into a local functional vector,
\begin{equation} \label{eq:functional}
    \bm{m}_f^{(t)} = \sigma_2~(\mbox{NN}_3~(\bm{h}^{(t)}; ~\bm{W}_3)).
\end{equation}

Each entry of $\bm{m}_f^{(t)}$ quantifies the significance of the corresponding functionality. Therefore, $\bm{m}_f^{(t)}$ can be viewed as an  anti-disease functionality combination for the current patient, $\bm{h}^{(t)}$. Next, we are motivated to generate the recommendation of drugs
that can cover all these anti-disease functionalities, while considering to prevent DDI between interacted drug pairs.

We therefore perform network pruning and design a novel masked neural network, $\mbox{NN}_4(\cdot): \mathbb{R}^{|\mathcal{S}|}
\mapsto \mathbb{R}^{|\mathcal{M}|}$, with $\bm{H}$ as the mask on network architecture. During the training process, $\mbox{NN}_4(\cdot)$ will learn to map the functionality vector $\bm{m}_f^{(t)}$ into the corresponding local drug representation,
\begin{align} \label{eq:mask}
\bm{m}_l^{(t)} =
\mbox{NN}_4~(\bm{m}_f^{(t)}; ~\mbox{MASK}~(\bm{W}_4, \bm{H})). 
\end{align}

We show that the mask $\bm{H}$ would enable the model to (i) have far fewer parameters (due to the sparsity of $\bm{H}$); (ii) prevent DDIs by avoiding a co-prescription of interacted drugs (we demonstrate it in the experiment section~\ref{sec:case1}).
% sending competing signals to interacted pair of drugs (we demonstrate it by a case study in the experiment).

% The bipartite embedding module is initially
% a standard fully connected network, and we substitute the
% last layer with sparse but informative bipartite structure $H$. This design aims
% at encoding drug dependencies, especially DDIs, directly into the model
% architecture, which enables the model to first identify required
% functionalities and then maps the functionalities to specific drug combinations. The
% motivation is that an ideal recommendation would be the combination of drugs
% that can cover all the anti-disease functionalities. In terms of pharmacology,
% it is the sub-structures of the molecule that determine what functionality the
% drugs could have and whether a pair of drugs would interact (and thus cause
% DDIs). Therefore, we superpose the bipartite structure in the last layer for
% better model intepretability and efficiency in preventing DDIs.

% To summarize, this module could be written as the following two steps. First, an
% $\mbox{NN}_3(\cdot)$ is applied for dimensionality transformation from
% $h^t$ to functional representation $m_f^t$. Then, another neural network
% $\mbox{NN}_4(\cdot)$, with bipartite mask $H$, transforms $m_f^t$ into local
% representation, $m_l^t$, \begin{align} m_f^t &= \mbox{NN}_3(h^t; ~W_3), \\ m_l^t &=
% \mbox{NN}_4(m_f^t; ~\mbox{MASK} (W_4, H)). \end{align}


\subsection{Medication Representation} 

The final medication representation is
given by treating the global drug matching vector as attention signals to further adjust
the local drug functionality representation. We further put an activation function $\sigma_3(\cdot)$ to scale the output,
\begin{equation}\label{eq:final} \hat{\bm{o}}^{(t)} = \sigma_3~(\bm{m}_g^{(t)} \odot \bm{m}_l^{(t)}), \end{equation}
where $\odot$ represents the element-wise product. By a threshold value
$\delta$, we can achieve the recommended drug combination, i.e., a multi-hot vector
$\hat{\bm{m}}^{(t)}$, by picking those entries where the value is greater than $\delta$. 


\subsection{Model Training and Inference} 

\method is trained end-to-end. We simultaneously learn the following parameters: the
diagnosis/procedure embedding tables $\bm{E}_d$, $\bm{E}_p$, parameters in $\mbox{RNN}_d$
and $\mbox{RNN}_p$, network parameters $\bm{W}_1$, atom embedding table $\bm{E}_a$,
layer-wise parameters in MPNN $\{\bm{W}^{(i)}\}$, affine parameters in LN, parameters
$\bm{W}_2$, $\bm{W}_3$ and $\bm{W}_4$.


\smallskip
\noindent
\textbf{Multiple Loss.} In this paper, the recommendation task is
formulated as multi-label  binary  classification. Suppose
$|\mathcal{M}|$ is the total number of drugs. We use $\bm{m}^{(t)}$ to denote the target
multi-hot drug recommendation, 
$\hat{\bm{o}}^{(t)}$ for the output real-valued drug representation (opposed to the predicted multi-hot vector $\hat{\bm{m}}^{(t)}$ after applying threshold $\delta$). We consider the
prediction of each drug as a sub-problem and use binary cross entropy
(BCE) as a loss, 
\begin{equation} \label{eq:bce} L_{bce} =
-\sum_{i=1}^{|\mathcal{M}|} \bm{m}^{(t)}_i log (\hat{\bm{o}}^{(t)}_i) + (1-\bm{m}^{(t)}_i)log (1-\hat{\bm{o}}^{(t)}_i),
\end{equation} where $\bm{m}^{(t)}_i$ and $\hat{\bm{o}}^{(t)}_i$ are the $i$-{th} entries. To make the
result more robust, we also adopt multi-label hinge loss to ensure
that the truth labels have at least 1 margin larger than others,
\begin{equation} \label{eq:multi}
L_{multi} = \sum_{i,j:~\bm{m}^{(t)}_i=1,\bm{m}^{(t)}_j= 0}
\frac{\mbox{max}(0,1-(\hat{\bm{o}}^{(t)}_i-\hat{\bm{o}}^{(t)}_j))}{|\mathcal{M}|}. \end{equation}
Based on the DDI adjacency matrix $\bm{D}$, we also design the adverse DDI loss over $\hat{\bm{o}}^{(t)}$ as, 
\begin{equation}  \label{eq:ddi}
L_{ddi} =
\sum_{i=1}^{|\mathcal{M}|}\sum_{j=1}^{|\mathcal{M}|} \bm{D}_{ij} \cdot \hat{\bm{o}}^{(t)}_i
\cdot \hat{\bm{o}}^{(t)}_j. \end{equation}
Note that the above loss functions are defined
for a single visit.  During the training, loss back propagation will be conducted at patient level by the averaged losses of this patient's all visits.

\smallskip
\noindent
\textbf{Controllable Loss Function.} A standard approach to training with
multiple loss functions is by weighted sum of the loss measuring terms
\cite{dosovitskiy2019you}, 
\begin{equation}  \label{eq:alpha}
L = \beta\left(\alpha L_{bce} +
(1-\alpha)L_{multi}\right) + \left(1-\beta\right)L_{ddi}, \end{equation} where $\alpha$ and
$\beta$ are usually pre-defined hyperparameters. 

In this scenario, two prediction
loss, $L_{bce}$ and $L_{multi}$, are compatible, and thus we select $\alpha$
from validation set. We observe that adverse DDIs also exist in the dataset
(doctors might mistakenly prescribe the interacted drugs). Therefore, by training with ground truth labels,
the correct learning process might conversely increase DDI. We therefore
consider to adjust $\beta$ during the training process by a
proportional–integral–derivative  (PID) controller \cite{an2018pid} to balance the prediction
loss and DDI loss. For simplicity, we only utilize the proportional error signal as negative feedback when DDI rate of the recommended drugs is above certain thresholds.

In safe drug recommendation, the key is to maintain a low DDI, so we set a DDI
acceptance rate $\gamma \in (0,1)$ for the loss function.
Our motivation is that if the patient-level DDI is lower than the threshold, $\gamma$, then we consider only maximizing the accuracy; otherwise, $\beta$ will adjust adaptively to minimize DDI as well.
% \js{Is there a citation for PID? What is the intuition for PID and what is PID solving for our problem. }

The controllable
factor $\beta$ follows the piece-wise strategy, \begin{equation}\label{eq:loss}
\beta =\left\{ \begin{array}{lr} 1, ~~& \mbox{DDI} \leq \gamma \\ \max~\{0, ~1 -
\frac{DDI - \gamma}{K_p}\}, ~~& \mbox{DDI} > \gamma \end{array} \right.
\end{equation}
where $K_p$ is a correcting factor for the proportional
signal. %
% In the extreme case, $\beta_{min}=1+\frac{\gamma-1}{K_p}~\mbox{or}~0$ when
% every pair of drugs in the combination do interact.

We show in the experiment that $\gamma$ can be viewed approximately as an upper bound of the
output DDI rate. By employing the PID controller and presetting different $\gamma$, our \method model
could provide reliable drug combinations to meet different level of DDI
requirements.

We summarize the procedure of one training epoch of our model in Algo.~\ref{algo:safedrug}. From {\em Line1} to {\em Line3}, we input some data sources, initialize the parameters by random $Uniform(-0.1, 0.1)$ distribution, and generate a bipartite mask $\bm{H}$ directly from the fragmentation result. From {\em Line4} to {\em Line8}, we select one patient from the training set and enumerate her/his clinical visits. In {\em Line9}, we embed the longitudinal diagnosis and procedure information into a patient representation, $\bm{h}^{(t)}$. Note that, our algorithm would store the hidden representation, $\bm{d}_h^{(t)}$ and $\bm{p}_h^{(t)}$ for the next visit. In {\em Line10} and {\em Line11}, we generate the global and local drug vector by MPNN encoder and bipartite encoder. We combine these two vectors in {\em Line12} and compute losses and conduct gradient descent in {\em Line14 and Line 15}.

\begin{algorithm}[h!]\small
 \SetAlgoLined
 \textbf{Input:} Training set $\mathcal{T}$, hyperparameters $\alpha, K_p$, pre-defined acceptance DDI rate $\gamma$ in Eqn.~\eqref{eq:alpha} and \eqref{eq:loss}, DDI matrix $\bm{D}$\;
 Initialize parameters: $\bm{E}_d,\bm{E}_p,\bm{E}_a,\mbox{RNN}_d, \mbox{RNN}_p, \bm{W}_i,\{\bm{W}^{(i)}\},\mbox{LN}$\;
 Obtain the bipartite mask, $\bm{H}$, by BRICS fragmentation \cite{degen2008art}\;
 \For{patient $j$ := 1 to $|\mathcal{T}|$}{
    Select the patient $j$'s history, $\bm{X}_j$ \;
    Obtain the global drug memory, $\bm{E}_g$, in Eqn.~\eqref{eq:z_i}, \eqref{eq:y_i} and \eqref{eq:y}\;
    \For{visit $t$ := 1 to $|\bm{X}_j|$}{
    Select the $t$-th visit of patient $j$, $\bm{x}_j^{(t)}$\;
    Generate embeddings, $\bm{d}_e^{(t)},\bm{p}_e^{(t)}$, in Eqn.~\eqref{eq:diag-emb}, \eqref{eq:prod-emb}; hidden representations, $\bm{d}_h^{(t)},\bm{p}_h^{(t)}$, in
    Eqn.~\eqref{eq:hidden-diag}, \eqref{eq:hidden-prod};
    and patient representation, $\bm{h}^{(t)}$, in Eqn.~\eqref{eq:patient_rep} // Patient Representation\;
    Generate matching vector, $\bm{m}_r^{(t)}$, and global drug vector, $\bm{m}_g^{(t)}$, from Eqn.~\eqref{eq:relevant} and \eqref{eq:global} // MPNN Encoder\;
    Generate functional vector, $\bm{m}_f^{(t)}$, and local drug vector, $\bm{m}_l^{(t)}$, from Eqn.~\eqref{eq:functional} and \eqref{eq:mask} // Bipartite Encoder\;
    Generate drug representation, $\hat{\bm{o}}_l^{(t)}$, and multi-hot drug vector, $\hat{\bm{m}}^{(t)}$, from Eqn.~\eqref{eq:final} // Drug Representation\;
 }
 Calculate $L_{bce},L_{multi},L_{ddi}$ in Eqn.~\eqref{eq:bce}, \eqref{eq:multi}, \eqref{eq:ddi}\;
    Choose $\beta$ and Optimizing the loss in Eqn.~\eqref{eq:alpha}, \eqref{eq:loss}\; 
 }
 \caption{One Training Epoch of \method}
 \label{algo:safedrug}
 %\vspace{-1mm}
\end{algorithm}




Model inference phase basically follows the same pipeline as training. We apply a threshold $\delta=0.5$ on the output drug representation in Eqn.~\eqref{eq:final} and collect drugs, corresponding to entries where the value is greater than $\delta$, as the final recommendations.



==> cover_letter/preliminaries.tex <==

\section{Problem Formulation} \label{sec:notation}

In this section, we list notations used in the paper  in Table~\ref{tb:notations} and formulate the safe drug recommendation problem.

\begin{table}[h!] \small \caption{Notations used in \method}
\centering
\resizebox{\columnwidth}{!}{
	\begin{tabular}{c|l} \toprule \textbf{Symbols} & \textbf{Descriptions} \\ 
	\midrule 
	$\bm{X}_j$ & EHR history of patient $j$ \\
	$\bm{x}^{(i)}_j$ & EHR record of patient $j$ at the $i$-th visit \\
	$V_j$ & total number of observed visits of patient $j$ \\
	$\bm{d}_j^{(i)},\bm{p}_j^{(i)},\bm{m}_j^{(i)}$ & diag./proc./med. vector of patient $j$ at the $i$-th visit\\
	$\mathcal{D}, \mathcal{P}, \mathcal{M}$ & overall diagnosis/procedure/medication code set \\
	$\bm{D}$ & binary DDI matrix \\
	$\bm{d}^{(t)},\bm{p}^{(t)},\bm{m}^{(t)}$ & a generic multi-hot diag./proc./med. vector at the $t$-th visit\\
	$\bm{E}_d, \bm{E}_p$ & diagnosis/procedure code embedding table \\
	$\bm{d}_e^{(t)},\bm{p}_e^{(t)}$ & a generic diag./proc. embedding vector at the $t$-th visit\\
	$\bm{d}_h^{(t)},\bm{p}_h^{(t)}$ & a generic diag./proc. hidden vector at the $t$-th visit\\
	$\bm{h}^{(t)}$ & a generic patient representation at the $t$-th visit\\
	$\bm{z}_i^{(l+1)}$ & messages from neighbors for atom $i$ at the $l$-th iteration \\
	$y_i^{(l+1)}$ & hidden state of atom $i$ at the $(l+1)$-th iteration \\
	$\bm{E}_a, \bm{E}_g$ & atom embedding table, global drug memory \\
	$\bm{m}^{(t)}_r, \bm{m}^{(t)}_g$ & matching vector and global drug vector at the $t$-th visit \\
	$\bm{m}^{(t)}_f, \bm{m}^{(t)}_l$ & functional vector and local drug vector at the $t$-th visit \\
	$\mathcal{C}$ & overall atom set \\
	$\bm{H}$ & bipartite mask matrix \\
	$\mathcal{S}$ & molecule substructure set \\
	$\hat{\bm{o}}^{(t)},\hat{\bm{m}}^{(t)}$ &predicted real-valued/multi-hot med. vector at the $t$-th visit\\
	$\mbox{NN}_i(\cdot)$ & feedforward neural networks \\
	$\bm{W}_i$ & weight matrices \\
	$\sigma_i(\cdot)$ & activation functions \\
	$\alpha,\beta,\gamma,K_p$ & (hyper)parameters in controllable loss function\\
    \bottomrule 
    \end{tabular}}
	\label{tb:notations} \end{table}


\begin{definition}[\textbf{Patient Electrical health records (EHR) Data}]
Patient EHR data
captures comprehensive medical histories of patients in the format of  longitudinal vectors of medical codes (e.g., diagnoses, procedures and drugs).
Formally, EHR for patient $j$ can be represented as a sequence $\bm{X}_j=[\bm{x}_j^{(1)},\bm{x}_j^{(2)},\dots,\bm{x}_j^{(V_j)}]$, where $V_j$ is the total number of
 visits for patient $j$. The $i$-th entry of $\bm{X}_j$ documents the $i$-th visit of patient $j$, specified by $\bm{x}_j^{(i)} = [\bm{d}_j^{(i)}, \bm{p}_j^{(i)}, \bm{m}_j^{(i)}]$, where $\bm{d}_j^{(i)}\in\{0,1\}^{|\mathcal{D}|}, \bm{p}_j^{(i)}\in\{0,1\}^{|\mathcal{P}|},\bm{m}_j^{(i)}\in\{0,1\}^{|\mathcal{M}|}$, are multi-hot diagnosis,
procedure and medication vectors, respectively. $\mathcal{D}, \mathcal{P}, \mathcal{M}$
are the corresponding element sets, and $|\cdot|$
denotes the cardinality. 
% For example, if patient $j$ received diagnoses with codes 3601, 3893,
% and 9915 in the $i$-th visit. Then, $\bm{d}_j^{(i)}$ would be a  $|\mathcal{D}|$-dim multi-hot vector, where three corresponding
% entries are 1s and the others are all 0s.

\end{definition} 

\begin{problem}[\textbf{Safe Drug Combination Recommendation}]

We focus on drug recommendation while reducing/controlling the drug-drug interaction (DDI) rates in the prediction.

For DDI, we use a symmetric binary adjacency matrix $\bm{D}\in
\{0,1\}^{|\mathcal{M}|\times|\mathcal{M}|}$ to denote DDI relation.
$\bm{D}_{ij}=1$ means that the
interaction between drug $i$ and $j$ has been reported while $\bm{D}_{ij}=0$
indicates a safe co-prescription.

Then for each patient, given the patient's up-to-now diagnosis and procedure sequences $[\bm{d}^{(1)}, \bm{d}^{(2)},
\dots, \bm{d}^{(t)}]$ and $[\bm{p}^{(1)}, \bm{p}^{(2)},
\dots, \bm{p}^{(t)}]$, the DDI matrix $\bm{D}$, the paper aims at learning a function, $f(\cdot)$, mapping from two medical sequences
% $[\bm{d}^{(i)}]_{i=1}^t, [\bm{p}^{(i)}]_{i=1}^t$, 
to a drug recommendation, $\hat{\bm{m}}^{(t)}\in
\{0,1\}^{|\mathcal{M}|}$. Specifically,
\begin{equation}
    \hat{\bm{m}}^{(t)} = f~([\bm{d}^{(i)}]_{i=1}^t, [\bm{p}^{(i)}]_{i=1}^t),
\end{equation} where the objective function consists of two parts: (i) extracting real drug combinations, $\bm{m}^{(t)}$, as supervision to penalize $\hat{\bm{m}}^{(t)}$; (ii) using matrix $\bm{D}$ to derive unsupervised DDI constraints on $\hat{\bm{m}}^{(t)}$.
\end{problem} 
% transforming $\hat{\bm{o}}^{(t)}$ into a multi-hot vector $\hat{\bm{m}}^{(t)}\in\{0,1\}^{|\mathcal{M}|}$ for

% \js{We should formally specify to learn a function mapping some input to a desirable output. The objective function with constraints should be specified.  Right now it looks vague and informal. }

==> cover_letter/relatedwork.tex <==
\section{Related Works}


% \cx{the paragraph below is copied from my previous paper. please modify/rephrase}

% \subsubsection{Medication Combination Recommendation and merge into section 2.1}
% could be categorized into instance-based and longitudinal medication recommendation methods. Instance-based methods focus on current health conditions. Among them, Leap~\cite{zhang2017leap} formulates a multi-instance multi-label learning framework and proposes a variant of sequence-to-sequence model based on content-attention mechanism to predict combination of medicines given patient's diagnoses. Longitudinal-based methods leverage the temporal dependencies among clinical events, see ~\cite{choi2016retain,choi2016doctor,lipton2015learning,le2018dual,doi:10.1093/jamia/ocy068}. Among them, RETAIN~\cite{choi2016retain} is based on a two-level neural attention model which detects influential past visits and significant clinical variables within those visits. DMNC~\cite{le2018dual} highlighted the memory component to enhance the memory ability of recurrent neural networks and combined DNC with RNN encoder-decoder to predict medicines based on patient's history records which has shown high accuracy. However, safety issue is often ignored by longitudinal-based methods. In this work, we design a memory component but target at building a structured graph augmented memory, where we not only embed DDI knowledge but also design a DDI loss to reduce DDI rate.


\subsection{Medication Recommendation} 
% The research of drug recommendation is developed from rule-based methods \cite{almirall2012designing,chen2016physician,lakkaraju2017learning}, where human-crafted features were labor-intensive for specific diagnoses. 
% With larger EHR data, supervised learning algorithms
% \cite{zhang2014towards,bajor2016predicting}, such as knowledge graph embedding
% \cite{wang2017safe,mao2019medgcn} became popular. 
Existing medication recommendation algorithms could be mainly categorized into instance-based and longitudinal recommendation methods. Instance-based approaches focus on patient's current health status. For example, LEAP \cite{zhang2017leap} extracts feature information from the current encounter and adopts a multi-instance multi-label setting for drug recommendation. Longitudinal approaches are proposed to leverage the temporal dependencies within the clinical history, see ~\cite{choi2016doctor,lipton2015learning,le2018dual,xiao2018opportunities}. Among them, RETAIN \cite{choi2016retain} utilizes a two-level RNN with reverse time attention to model the longitudinal information. DMNC \cite{le2018dual} builds on differentiable neural computer (DNC) and uses a memory component to enhance the multi-view RNN modeling. GAMENet \cite{shang2019gamenet} adopts memory augmented neural networks (MANN) and stores historical drug information as references for further prediction. These methods either model the final drug combination as multi-label binary classification \cite{choi2016retain,shang2019gamenet,shang2019pre} or by sequential decision making \cite{zhang2017leap,wang2019order,le2018dual}. Despite their initial success, these existing works still have the following limitations.
There are other important data such as {\em drug molecule structures}  which can help augment drug recommendation but have not been utilized by existing models. Also, existing works  model DDI inadequately, either via soft or indirect constraints. 

In this paper, we propose a DDI-controllable drug recommendation model  that not only leverages drugs' molecule structures but also models DDIs effectively.



\subsection{Molecule Representation}
Molecule graph representation remains an important topic  due to the association between molecule structure and their properties, e.g., efficacy and safety.  
Early days,  molecular
descriptors~\cite{mauri2006dragon,steinbeck2003chemistry} and
drug fingerprint~\cite{glen2006circular,rogers2010extended,duvenaud2015convolutional} were commonly used to represent drug molecules.
Recent years, deep learning models were developed to learn molecule representation and model molecule substructures (a set of connected atoms). For example, \cite{huang2020caster} developed a
sequential pattern mining method on SMILES strings and modeled a pair of drugs as a set of their substring representation. In addition, \cite{huang2020deeppurpose}
proposed to directly model molecule graphs using graph-based neural network models ~\cite{tang2020self,you2018graph}. 


In this paper, inspired by \cite{huang2020caster,huang2020deeppurpose}, \method is proposed to capture both the molecular global and local information during  the recommendation. The paper adopts a novel graph-based encoder with learned initial fingerprints to model the molecule, as global property is essential. The model also segments molecules into local substructures, which associate with useful functional groups.

